Case study of SARS-CoV-2 transmission risk assessment in indoor environments using cloud computing resources

Complex flow simulations are conventionally performed on HPC clusters. However, the limited availability of HPC resources and steep learning curve of executing on traditional supercomputer infrastructure has drawn attention towards deploying flow simulation software on the cloud. We showcase how a complex computational framework -- that can evaluate COVID-19 transmission risk in various indoor classroom scenarios -- can be abstracted and deployed on cloud services. The availability of such cloud-based personalized planning tools can enable educational institutions, medical institutions, public sector workers (courthouses, police stations, airports, etc.), and other entities to comprehensively evaluate various in-person interaction scenarios for transmission risk. We deploy the simulation framework on the Azure cloud framework, utilizing the Dendro-kT mesh generation tool and PETSc solvers. The cloud abstraction is provided by RocketML cloud infrastructure. We compare the performance of the cloud machines with state-of-the-art HPC machine TACC Frontera. Our results suggest that cloud-based HPC resources are a viable strategy for a diverse array of end-users to rapidly and efficiently deploy simulation software.

==> Data/comparDendro4Table.tex <==
{\renewcommand{\arraystretch}{1.1} %<- modify value to suit your needs
\begin{table}[t!]
\resizebox{\linewidth}{!}{%
{
\Large
\begin{tabular}{|c|c|c|r|r|r|r|r|}
\hline
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{Base} \\ \textbf{Refinement}\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{Boundary} \\ \textbf{Refinement}\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{Num} \\ \textbf{Elements}\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{Num}\\ \textbf{Processors}\end{tabular}} & \multicolumn{2}{c|}{\textbf{\Dendro{} (s)}} & \multicolumn{2}{c|}{\textbf{Current Approach (s)}} \\ \cline{5-8} 
 &  &  &  & \begin{tabular}[c]{@{}c@{}}Mesh\\Creation\end{tabular} & \mvec{} & \begin{tabular}[c]{@{}c@{}}Mesh\\Creation\end{tabular} & \mvec{} \\ \hline
\multirow{3}{*}{10} & \multirow{3}{*}{12} & \multirow{3}{*}{3,138,525} & 448 & 107.87 & 59.14 & 1.69 & 9.27 \\ \cline{4-8} 
 &  &  & 896 & 55.41 & 38.03 & 1.00 & 4.53 \\ \cline{4-8} 
 &  &  & 1792 & 38.21 & 25.47 & 0.87 & 2.34 \\ \hline
\multirow{3}{*}{10} & \multirow{3}{*}{14} & \multirow{3}{*}{49,096,209} & 448 & 280.88 & 447.05 & 21.51 & 142.89 \\ \cline{4-8} 
 &  &  & 896 & 159.87 & 349.39 & 11.51 & 77.33 \\ \cline{4-8} 
 &  &  & 1792 & 127.21 & 295.02 & 6.34 & 48.51 \\ \hline
\multirow{3}{*}{12} & \multirow{3}{*}{12} & \multirow{3}{*}{17,440,929} & 448 & - & - & 4.57 & 42.58 \\ \cline{4-8} 
 &  &  & 896 & - & - & 2.29 & 19.65 \\ \cline{4-8} 
 &  &  & 1792 & - & - & 1.75 & 10.76 \\ \hline
\multirow{3}{*}{12} & \multirow{3}{*}{14} & \multirow{3}{*}{63,398,613} & 448 & - & - & 33.56 & 182.23 \\ \cline{4-8} 
 &  &  & 896 & - & - & 17.14 & 125.53 \\ \cline{4-8} 
 &  &  & 1792 & - & - & 9.86 & 47.65 \\ \hline
\end{tabular}
}
}
\vspace{5mm}
\caption{\footnotesize{Comparison of the time (in seconds) for mesh generation and Navier--Stokes \mvec{} for the current approach with \Dendro{} based octree framework. With level $\geq$ 12 of base refinement, ~\Dendro~ framework gave memory error, and hence no time is reported.}}
\label{tab:comparDendro4}
\end{table}
}

==> Data/ibmComparD5.tex <==
\added{
{\renewcommand{\arraystretch}{1.4} %<- modify value to suit your needs
\begin{table}[t!]
\resizebox{0.99\linewidth}{!}{%
{
\Large
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|}
\hline
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{Base}\\ \textbf{level}\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{Exit} \\ \textbf{refine}\\ \textbf{level}\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{Body}\\ \textbf{refine}\\ \textbf{level}\end{tabular}} & \multicolumn{2}{c|}{\textbf{Elements}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{Num} \\ \textbf{procs}\end{tabular}} & \multicolumn{2}{c|}{\textbf{Immersed (s)}} & \multicolumn{2}{c|}{\textbf{Carved out (s)}} \\ \cline{4-5} \cline{7-10} 
 &  &  & \begin{tabular}[c]{@{}c@{}}\textbf{Active} \\ \textbf{Elements}\end{tabular} & \begin{tabular}[c]{@{}c@{}}$f_{\mathrm{excess}}$ \end{tabular} &  & \begin{tabular}[c]{@{}c@{}}\textbf{Mesh} \\ \textbf{construction}\end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{Solve}\\ \textbf{time}\end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{Mesh} \\ \textbf{construction}\end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{Solve}\\ \textbf{time}\end{tabular} \\ \hline
\multirow{2}{*}{6} & \multirow{2}{*}{8} & \multirow{2}{*}{10} & \multirow{2}{*}{924,549} & \multirow{2}{*}{1.53} & 224 & 92.36 & 178.74 & 38.57 & 61.56 \\ \cline{6-10} 
 &  &  &  &  & 448 & 50.48 & 94.95 & 22.47 & 32.05 \\ \hline
\multirow{2}{*}{6} & \multirow{2}{*}{9} & \multirow{2}{*}{10} & \multirow{2}{*}{1,259,670} & \multirow{2}{*}{1.43} & 224 & 136.13 & 220.6 & 48 & 83.3 \\ \cline{6-10} 
 &  &  &  &  & 448 & 73.24 & 95.06 & 28.88 & 45.10 \\ \hline
\multirow{2}{*}{7} & \multirow{2}{*}{9} & \multirow{2}{*}{11} & \multirow{2}{*}{3,461,548} & \multirow{2}{*}{1.64} & 448 & 210.8 & 309.60 & 89.04 & 131.52 \\ \cline{6-10} 
 &  &  &  &  & 896 & 107.88 & 161.70 & 53.24 & 71.3 \\ \hline
\end{tabular}
}
}
\vspace{0.2in}
\caption{\added{\footnotesize{Comparison of mesh generation and solve time for IBM  with the current approach for the classroom case. The carved out approach leads to a significant reduction in number of elements. $f_{\mathrm{excess}}$ represents the excess fraction of elements obtained as a result of generating complete octree. \vspace{-5 mm}}}}
\label{tab:comparD5}
\end{table}
}
}

==> Data/scalCompar.tex <==
{\renewcommand{\arraystretch}{1.1} %<- modify value to suit your needs
\begin{table}[t!]
\resizebox{\linewidth}{!}{%
{
\Large
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Case\\ Type\end{tabular}}} & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Element\\ Order\end{tabular}}} & \multicolumn{3}{c|}{\textbf{Strong scaling}} & \multicolumn{2}{c|}{\textbf{Weak Scaling}} \\ \cline{3-7} 
 &  & \textbf{\begin{tabular}[c]{@{}c@{}}Num \\ elements\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Num\\ DOFs\end{tabular}} & \textbf{Efficiency} & \textbf{\begin{tabular}[c]{@{}c@{}}Num \\ elements/core\end{tabular}} & \textbf{Efficiency} \\ \hline
\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Channel\\ (\secref{sec:channelScaling})\end{tabular}}} & \textbf{Linear} & 13.5 M & 13.7 M & 0.81 & 35K & 0.82 \\ \cline{2-7} 
 & \textbf{Quadratic} & 13.5 M
 & 101.9 M & 0.90 & 35K & 0.86 \\ \hline
\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Sphere\\ (\secref{sec:sphereScaling})\end{tabular}}} & \textbf{Linear} & 17.5 M & 17.4 M & 0.90 & 10K & 0.74 \\ \cline{2-7} 
 & \textbf{Quadratic} & 17.5 M & 139.7 M & 0.96 & 10K & 0.83 \\ \hline
\end{tabular}
}
}
\vspace{5 mm}
\caption{\added{\footnotesize{Summary of scaling efficiency for the channel and spherical carved out region.}}}
\label{tab:scalCompar}
\end{table}
}

==> Data/tabDofCompar.tex <==
\added{
{\renewcommand{\arraystretch}{1.1} %<- modify value to suit your needs
\begin{table}[t!]
%\resizebox{\linewidth}{!}
{%
\footnotesize
{
\begin{tabular}{|c|c|c|c|c|c|}
\hline
\multicolumn{2}{|c|}{\multirow{2}{*}{}} & \multicolumn{4}{c|}{Refine Level} \\ \cline{3-6} 
\multicolumn{2}{|c|}{}  & 11 & 12 & 13 & 14 \\ \hline
\multirow{2}{*}{Sphere} & $f_{\text{elem}}$ & 1.75 & 1.79 & 1.81 & 1.82 \\ \cline{2-6} 
 & $f_\text{DOF}$ & 1.30 & 1.31 & 1.32 & 1.33 \\ \hline
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Stanford\\ Dragon\end{tabular}} & $f_{\text{elem}}$ & 1.84 & 1.87 & 1.90 & 1.92 \\ \cline{2-6} 
 & $f_\text{DOF}$ & 1.36 & 1.39  & 1.41 & 1.43 \\ \hline
\end{tabular}
}
}
\vspace{5mm}
\caption{\added{\footnotesize{Comparison of the ratio of number of elements ($f_\text{elem}$) and degrees of freedom ($f_\text{DOF}$) with and without (\textit{immersed}) carving out the sphere and the Stanford dragon from the domain. The base refinement was set to 4 and the refinement level near the object was varied from 11 to 14.}}}
% \vspace{-0.3in}
\label{tab:dofCompar}
\end{table}
}
}

==> Data/tabScalingClassroom.tex <==
\added{
{\renewcommand{\arraystretch}{1.3} %<- modify value to suit your needs
\begin{table}[t!]
\resizebox{\linewidth}{!}{%
{
\Large
\begin{tabular}{|c|c|c|c|c|c|c|c|c|l|}
\hline
\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Base \\ level\end{tabular}}} & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Exit\\ level\end{tabular}}} & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Body \\ Level\end{tabular}}} & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Num \\ Elements\end{tabular}}} & \multirow{2}{*}{\textbf{}} & \multicolumn{5}{c|}{\textbf{Number of Processors}} \\ \cline{6-10} 
 &  &  &  &  & 224 & 448 & 896 & 1792 & 3584 \\ \hline
\multirow{2}{*}{7} & \multirow{2}{*}{8} & \multirow{2}{*}{11} & \multirow{2}{*}{5,555,871} & {Time(s)} & 344.87 & 176.15 & 92.16 & 46.44 & 23.95 \\ \cline{5-10} 
 &  &  &  & {Efficiency} & 1.0 & 0.98 & 0.94 & 0.93 & 0.90 \\ \hline
\multirow{2}{*}{9} & \multirow{2}{*}{9} & \multirow{2}{*}{11} & \multirow{2}{*}{23,054,077} & {Time(s)} & - & 539.15 & 272.28 & 142.73 & 75.7 \\ \cline{5-10} 
 &  &  &  & {Efficiency} & - & 1.0 & 0.99 & 0.94 & 0.89 \\ \hline
\end{tabular}
}
}
\vspace{0.2in}
\caption{\added{\footnotesize{\textit{Scaling result for classroom simulation:} Comparison of total solve time and strong scaling efficiency with increase in processor count for two different meshes with varying levels of refinement.}}\vspace{-2 mm}}
\label{tab:scalClassroom}
\end{table}
}
}


==> Data/tableConditionNumber.tex <==
\begin{table}[t!]
\newcommand{\tabincell}[2]{\begin{tabular}{@{}#1@{}}#2\end{tabular}}
\footnotesize
\begin{tabular}{|c|c|r|c|r|}
\hline
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Channel \\ length\end{tabular}} & \multicolumn{2}{c|}{Complete octree} & \multicolumn{2}{c|}{Incomplete octree} \\ \cline{2-5} 
 & DOFs & \tabincell{c}{Condition\\Number} & DOFs & \tabincell{c}{Condition\\Number} \\ \hline
1 & 1089 & 402.6 & 1089 & 402.6 \\ \hline
2 & 1089 & 466.7 & 561 & 155.6 \\ \hline
4 & 1089 & 510.1 & 297 & 42.5 \\ \hline
8 & 1089 & 512.0 & 165 & 13.3 \\ \hline
16 & 1089 & 10580.5 & 99 & 5.0 \\ \hline
\end{tabular}
\vspace{5 mm}
\caption{\footnotesize{Comparison of condition number for the case with complete octree and incomplete octree. In the case of complete octree, each element of the mesh was stretched according to the channel aspect ratio (represented here by the length) to conform with the channel boundaries, whereas in the case of incomplete octree, the aspect ratio was fixed to be 1 and the elements outside the domain are removed.}}
\label{table: conditionNumber}
\end{table}

==> Images/IntroFig.tex <==
\begin{figure}
\begin{subfigure}{0.4\linewidth}
\centering
    \begin{tikzpicture}[scale=0.4, transform shape]
     \fill[cpu1] (0.0,0.0) rectangle (7.5,7.5);
    % \fill[cpu1] (6.0,0.0) rectangle (7.5,6.0);
    \fill[cpu2] (0.75,4.5) rectangle (5.25,5.25);
    \fill[cpu2] (1.50,5.25) rectangle (4.5,6.0);
    \fill[cpu2] (0.75,0.75) rectangle (1.5,4.5);
    \fill[cpu2] (4.5,0.75) rectangle (5.25,4.5);
    \fill[cpu2] (0.0,1.5) rectangle (0.75,4.5);
    \fill[cpu2] (5.25,1.5) rectangle (6.0,4.5);
    \fill[cpu2] (1.50,0.0) rectangle (4.5,3.0);
    % \fill[cpu2] (1.50,5.25) rectangle (4.5,6.0);
    
    % \fill[cpu2] (0.0,0.0) rectangle (6.0,1.5);
    % \fill[cpu2] (0.0,1.5) rectangle (1.5,4.5);
    % \fill[cpu2] (4.5,1.5) rectangle (6.0,4.5);
    \fill[cpu4] (4.5,1.5) rectangle (1.5,4.5);
    \fill[cpu4] (0.75,2.25) rectangle (1.5,3.75);
    \fill[cpu4] (4.5,2.25) rectangle (5.25,3.75);
    \fill[cpu4] (2.25,4.5) rectangle (3.75,5.25);
    \fill[cpu4] (2.25,0.75) rectangle (3.75,1.5);
    \draw[step=1.5cm, thick] (0,0) grid (7.5,7.5);
    \draw[-,black, thick] (0,0.75) -- (6,0.75);
    \draw[-,black, thick] (0,5.25) -- (6,5.25);
    \draw[-,black, thick] (0.75,0) -- (0.75,6.0);
    \draw[-,black, thick] (5.25,0) -- (5.25,6.0);
    \draw[-,black, thick] (2.25,0) -- (2.25,1.5);
    \draw[-,black, thick] (3.75,0) -- (3.75,1.5);
    \draw[-,black, thick] (2.25,4.5) -- (2.25,6.0);
    \draw[-,black, thick] (3.75,4.5) -- (3.75,6.0);
    
    \draw[-,black, thick] (0,2.25) -- (1.5,2.25);
    \draw[-,black, thick] (0,3.75) -- (1.5,3.75);
    
    \draw[-,black, thick] (4.5,2.25) -- (6,2.25);
    \draw[-,black, thick] (4.5,3.75) -- (6,3.75);

    % \fill[gray,opacity = 0.4 ] (3,3 ) circle (2.5cm);
    \draw[red,ultra thick] (3,3 ) circle (2.5cm);
   
    % \fill[red,opacity = 0.2] (6.0,0.0) rectangle (7.5,6.0);
    \foreach \x in {0,1.5,...,7.5}{
            \draw [fill=red](\x,0.0) circle (0.1cm);
            \draw [fill=red](\x,7.5) circle (0.1cm);
            \draw [fill=red](\x,6.0) circle (0.1cm);
    }
    \foreach \y in {0,1.5,...,7.5}{
            \draw [fill=red](0.0,\y) circle (0.1cm);
            \draw [fill=red](6.0,\y) circle (0.1cm);
            \draw [fill=red](7.5,\y) circle (0.1cm);
    }
    
    \foreach \x in {1.5,3.0,4.5}
    \foreach \y in {1.5,3.0,4.5}
        \draw [fill=gray](\x,\y) circle (0.1cm);
        
    \foreach \y in {0.0,0.75,...,5.9}{
        \draw [fill=red](0.0,\y) circle (0.1cm);
        % \draw [fill=red](6.0,\y) circle (0.1cm);
        \draw [fill=red](0.75,\y) circle (0.1cm);
        \draw [fill=red](5.25,\y) circle (0.1cm);
    }
    \foreach \x in {0.0,0.75,...,5.9}{
        \draw [fill=red](\x,0.0) circle (0.1cm);
        \draw [fill=red](\x,0.75) circle (0.1cm);
        \draw [fill=red](\x,5.25) circle (0.1cm);
    }
    
    \foreach \x in {2.25,3.0,...,4.2}{
        \draw [fill=gray](\x,0.75) circle (0.1cm);
        \draw [fill=gray](\x,5.25) circle (0.1cm);
    }
    \foreach \y in {2.25,3.0,...,4.2}{
        \draw [fill=gray](5.25,\y) circle (0.1cm);
        \draw [fill=gray](0.75,\y) circle (0.1cm);
    }
    %  \draw [fill=none,color=black,ultra thick](3.0,3.0) circle (0.3cm);
    %  \draw [fill=none,color=black,thick](3.0,4.5) circle (0.3cm);
    %  \draw [fill=none,color=black,thick](3.0,1.5) circle (0.3cm);
    %  \draw [fill=none,color=black,thick](1.5,3.0) circle (0.3cm);
    %  \draw [fill=none,color=black,thick](4.5,3.0) circle (0.3cm);
    % % \fill[red,opacity = 0.2] (0.0,-0.9) rectangle (0.3,-0.6);
    % \node[align=left] at (1.5,-0.75) {\Intercepted};
    
    % \fill[blue,opacity = 0.2] (3.0,-0.9) rectangle (3.3,-0.6);
    % \node[align=left] at (4.5,-0.75) {\Out};
    
    % \fill[black,opacity = 0.2] (6.0,-0.9) rectangle (6.3,-0.6);
    % \node[align=left] at (6.7,-0.75) {\In};
    % % \fill[red,opacity = 0.2] (0.0,-0.9) rectangle (0.3,-0.6);
    % % \node at (1.5,-0.75) {\Intercepted};
    
    \end{tikzpicture}
    \caption{Complete quadtree}
    \label{fig: complete}
    \end{subfigure}
    \hspace{3 mm}
    \begin{subfigure}{0.4\linewidth}
    \centering
    \begin{tikzpicture}[scale=0.4, transform shape]
     \fill[cpu1] (0.0,0.0) rectangle (7.5,7.5);
    % \fill[cpu1] (6.0,0.0) rectangle (7.5,6.0);
    \fill[cpu2] (0.75,4.5) rectangle (5.25,5.25);
    \fill[cpu2] (1.50,5.25) rectangle (4.5,6.0);
    \fill[cpu2] (0.75,0.75) rectangle (1.5,4.5);
    \fill[cpu2] (4.5,0.75) rectangle (5.25,4.5);
    \fill[cpu2] (0.0,1.5) rectangle (0.75,4.5);
    \fill[cpu2] (5.25,1.5) rectangle (6.0,4.5);
    \fill[cpu2] (1.50,0.0) rectangle (4.5,3.0);
    % \fill[cpu2] (1.50,5.25) rectangle (4.5,6.0);
    
    % \fill[cpu2] (0.0,0.0) rectangle (6.0,1.5);
    % \fill[cpu2] (0.0,1.5) rectangle (1.5,4.5);
    % \fill[cpu2] (4.5,1.5) rectangle (6.0,4.5);

    \draw[step=1.5cm, thick] (0,0) grid (7.5,7.5);
    \draw[-,black, thick] (0,0.75) -- (6,0.75);
    \draw[-,black, thick] (0,5.25) -- (6,5.25);
    \draw[-,black, thick] (0.75,0) -- (0.75,6.0);
    \draw[-,black, thick] (5.25,0) -- (5.25,6.0);
    \draw[-,black, thick] (2.25,0) -- (2.25,1.5);
    \draw[-,black, thick] (3.75,0) -- (3.75,1.5);
    \draw[-,black, thick] (2.25,4.5) -- (2.25,6.0);
    \draw[-,black, thick] (3.75,4.5) -- (3.75,6.0);
  
    
    \draw[-,black, thick] (0,2.25) -- (1.5,2.25);
    \draw[-,black, thick] (0,3.75) -- (1.5,3.75);
    
    \draw[-,black, thick] (4.5,2.25) -- (6,2.25);
    \draw[-,black, thick] (4.5,3.75) -- (6,3.75);

    % \fill[gray,opacity = 0.4 ] (3,3 ) circle (2.5cm);
    \draw[red,ultra thick] (3,3 ) circle (2.5cm);
   
     
   
    \draw[-,white, ultra thick] (2.25,1.5) -- (3.75,1.5);
    \draw[-,white, ultra thick] (0.75,3.0) -- (5.25,3.0);
    \draw[-,white, ultra thick] (2.25,4.5) -- (3.75,4.5);
    % \fill[red,opacity = 0.2] (6.0,0.0) rectangle (7.5,6.0);
    \foreach \x in {0,1.5,...,7.5}{
            \draw [fill=red](\x,0.0) circle (0.1cm);
            \draw [fill=red](\x,7.5) circle (0.1cm);
            \draw [fill=red](\x,6.0) circle (0.1cm);
    }
    \foreach \y in {0,1.5,...,7.5}{
            \draw [fill=red](0.0,\y) circle (0.1cm);
            \draw [fill=red](6.0,\y) circle (0.1cm);
            \draw [fill=red](7.5,\y) circle (0.1cm);
    }
    

        
    \foreach \y in {0.0,0.75,...,5.9}{
        \draw [fill=red](0.0,\y) circle (0.1cm);
        % \draw [fill=red](6.0,\y) circle (0.1cm);
        \draw [fill=red](0.75,\y) circle (0.1cm);
        \draw [fill=red](5.25,\y) circle (0.1cm);
    }
    \foreach \x in {0.0,0.75,...,5.9}{
        \draw [fill=red](\x,0.0) circle (0.1cm);
        \draw [fill=red](\x,0.75) circle (0.1cm);
        \draw [fill=red](\x,5.25) circle (0.1cm);
    }
    
    
    %  \draw [fill=none,color=black,ultra thick](3.0,3.0) circle (0.3cm);
    %  \draw [fill=none,color=black,thick](3.0,4.5) circle (0.3cm);
    %  \draw [fill=none,color=black,thick](3.0,1.5) circle (0.3cm);
    %  \draw [fill=none,color=black,thick](1.5,3.0) circle (0.3cm);
    %  \draw [fill=none,color=black,thick](4.5,3.0) circle (0.3cm);
    % % \fill[red,opacity = 0.2] (0.0,-0.9) rectangle (0.3,-0.6);
    % \node[align=left] at (1.5,-0.75) {\Intercepted};
    
    % \fill[blue,opacity = 0.2] (3.0,-0.9) rectangle (3.3,-0.6);
    % \node[align=left] at (4.5,-0.75) {\Out};
    
    % \fill[black,opacity = 0.2] (6.0,-0.9) rectangle (6.3,-0.6);
    % \node[align=left] at (6.7,-0.75) {\In};
    % \fill[red,opacity = 0.2] (0.0,-0.9) rectangle (0.3,-0.6);
    % \node at (1.5,-0.75) {\Intercepted};
     % Cancelling internal nodes
     \fill[white] (4.5,1.5) rectangle (1.5,4.5);
    \fill[white] (0.75,2.25) rectangle (1.5,3.75);
    \fill[white] (4.5,2.25) rectangle (5.25,3.75);
    \fill[white] (2.25,4.5) rectangle (3.75,5.25);
    \fill[white] (2.25,0.75) rectangle (3.75,1.5);
    \fill[white] (2.25,0.75) rectangle (3.75,1.5);
    \fill[white] (0.75,2.25) rectangle (5.25,3.75);
    
    
     \foreach \y in {2.25,3.0,...,4.2}{
        \draw [fill=gray](5.25,\y) circle (0.1cm);
        \draw [fill=gray](0.75,\y) circle (0.1cm);
    }
    \foreach \x in {2.25,3.0,...,4.2}{
        \draw [fill=gray](\x,0.75) circle (0.1cm);
        \draw [fill=gray](\x,5.25) circle (0.1cm);
    }
   \draw [fill=gray](1.5,1.5) circle (0.1cm);
   \draw [fill=gray](2.25,1.5) circle (0.1cm);
   \draw [fill=gray](3.75,1.5) circle (0.1cm);
   \draw [fill=gray](4.5,2.25) circle (0.1cm);
   \draw [fill=gray](5.25,2.25) circle (0.1cm);
   \draw [fill=gray](4.5,1.5) circle (0.1cm);
   \draw [fill=gray](4.5,3.75) circle (0.1cm);
   \draw [fill=gray](1.5,1.5) circle (0.1cm);
   \draw [fill=gray](1.5,3.75) circle (0.1cm);
   \draw [fill=gray](1.5,4.5) circle (0.1cm);
   \draw [fill=gray](2.25,4.5) circle (0.1cm);
   \draw [fill=gray](3.75,4.5) circle (0.1cm);
   \draw [fill=gray](4.5,4.5) circle (0.1cm);
   \draw [fill=gray](1.5,2.25) circle (0.1cm);
    \end{tikzpicture}
    \caption{Incomplete quadtree}
    \label{fig: incomplete}
    \end{subfigure}
    \vspace{4 mm}
    \caption{
    A disk (enclosed region within the red circle) immersed in a \textit{complete} (~\figref{fig: complete}) or \textit{incomplete} (~\figref{fig: incomplete}) quadtree mesh.
    Every leaf in the tree represents an element occupying a region of space,
    which is either
    completely \textit{inside} (\textcolor{cpu4}{$\blacksquare$}) the body;
    completely \textit{outside} (\textcolor{cpu1}{$\blacksquare$}) the body;
    or \textit{intercepted} (\textcolor{cpu2}{$\blacksquare$}) by the boundary (solid red circle).
    A complete tree (\figref{fig: complete}) requires all $2^d$ children
    of each non-leaf subtree to be present,
    and thus gaps are not allowed in the middle of the mesh.
    However, useful information is only contributed by elements outside (\textcolor{cpu1}{$\blacksquare$}) or intercepted (\textcolor{cpu2}{$\blacksquare$}) by the body. \vspace{1 mm}
    % The present work extends tree-based FEM algorithms
    % to \textit{incomplete} trees (\figref{fig: incomplete}),
    % allowing subtrees inside the body to be carved out from the mesh,
    % and thus eliminated from FEM computations.
    % \secref{sec: Methods} formalizes the carving-out process
    % and explains how one may traverse incomplete trees to carry out FEM computations.
    %
    %     \figref{fig: incomplete} shows a incomplete octree carved out from the complete octree shown in ~\figref{fig: complete}.
    % The solid red line represents the boundary of the  immersed object. The elements are classified into 3 types:
    % a) \Out (\textcolor{cpu1}{$\blacksquare$}) : all nodes are outside the body;
    % b) \In (\textcolor{cpu4}{$\blacksquare$}): all nodes are inside the body;
    % c) \Intercepted (\textcolor{cpu2}{$\blacksquare$}) : some of the nodes are inside and some are outside. The hanging nodes are neither classified \In or \Out as they do not form independent degrees of freedom. In order to carve-out the the tree, (described in detail in ~\secref{sec: Methods}), we retain \Out and \Intercepted elements. All the \In nodes of \Intercepted elements forms a complete set of boundary nodes. Note that it is essential to ensure that none of the boundary nodes are hanging.
    % \mi{Polish this}
    } 
    \label{fig:carvedFig}
\end{figure}{}


==> OldFiles/Abstract.tex <==
% Efficiently and accurately simulating partial differential equations (PDEs) in and around arbitrarily defined geometries, especially with high levels of adaptivity, has significant implications for different application domains. A key bottleneck in the above process is the fast construction of a `good' adaptively-refined mesh. In this work, we present an efficient novel octree-based adaptive discretization approach capable of carving out arbitrarily shaped void regions from the parent domain: an essential requirement for fluid simulations around complex objects. Carving out objects produces an \textit{incomplete octree}.  We develop efficient top-down and bottom-up traversal methods to perform finite element computations on \textit{incomplete} octrees. We validate the framework by (a) showing appropriate convergence analysis and (b) computing the drag coefficient for flow past a sphere for a wide range of Reynolds numbers ($\mathcal{O}(1-10^6)$) encompassing the \emph{drag crisis} regime. Finally, we deploy the framework on a realistic geometry on a current project to evaluate COVID-19 transmission risk in classrooms.
 
%  %By leveraging the power of the mesh generator in conjunction with a finite element method (FEM) strategy for solving the Navier-Stokes equation, we showcase the method on three non - trivial applications (a) computing the drag coefficient for flow past a sphere for a wide range of Reynolds numbers ($\mathcal{O}(1-10^6)$) encompassing \emph{drag crisis} regime, (b) flow in a packed bed micro-channel, and (c) evaluating COVID-19 virus transmission risk under classroom conditions. 
 
%  %Traditional mesh-based finite element \mvec~ on adaptive grids require indirect memory accesses supported through neighborhood data structures. In contrast, our mesh-free approaches rely on top-down and bottom-up traversals on the grid leading to memory friendly computations. 

TODO

==> OldFiles/Applications.tex <==
This work is motivated by applications that requires adaptive octrees for discretizing long channels or complex geometries. In such cases, the traditional method of generating octree fails on account of their symmetric nature in all the dimension. Our target applications involve simulating the Navier--Stokes equations in three scenarios of increasing complexity: a) flow across a single complex object for a very wide range Reynolds numbers ($Re$); b) flow across a stack of identical objects representing a packed-bed biomedical microfluidic device; and c) flow across a stack of complex heterogeneous objects representing virus transmission in an occupied classroom. These canonical applications exemplify the difficulty of anisotropic geometries as well as presence of multiple complex objects in the simulation domain. %All these applications either have a long channel or complex objects or combination of both.

\subsubsection{LES simulation over complex objects}
Traditionally, unstructured body conforming grid was used to solve the Navier--Stokes equation over complex geometries. The generation of these analysis-suitable,  body-fitted mesh with appropriate refinement near the geometry is usually a time consuming and labor intensive process. Immersed boundary method (IBM) tends to alleviate these time consuming laborious process and no longer requires the body conforming meshes. In the past, we have successfully deployed Immersogeometric analysis (IMGA, IBM variant within FEM context), on a massively parallel octrees and shown the ability to capture the flow physics accurately \cite{saurabh2020industrial}. 

Although these methods have been shown to accurately capture the flow physics across a wide range of $Re$, they come at an additional cost of performing a surface loop over the geometry, to account for the immersed geometry ~\citep{saurabh2020industrial,xu2016tetrahedral,xu2019immersogeometric}. In order to successfully deploy IMGA, the surface discretization of the geometry must ensure that each background \Intercepted elements must contain at least 3-4 surface quadrature points. This overhead increases substantially with increase in the level of refinement of the background mesh and becomes a bottleneck especially for high $Re$ flow which inherently requires a very refine region close to the body in order to accurately capture the flow physics.  We refer the interested reader to ~\citet{saurabh2020industrial} for a detailed discussion on deployment of IMGA on octrees. We note that, with an increase in the refinement near the object, the voxelated \textit{carved} out geometry asymptotically approaches the actual geometry. As shown in \figref{fig: ProjectedArea} for a sphere, the projected area \footnote{Projected area is chosen as a measure at it plays an important role in determining the aerodynamic coefficient.} of the voxelated sphere asymptotically converges to the theoretical value. Thus, for applications where the inherent physics requires a fine resolution near the boundaries, e.g. the cases with thin boundary layers, using a \textit{carved} geometry becomes a viable choice to accurately perform the flow simulation.
\input{Plots/ProjectedArea}
\input{Plots/signedDistance}

\subsubsection{Lab on a chip devices}
With recent advances in fabrication process and 3D printing, high throughput microfluidic devices, capable of performing multiplexed laboratory analysis at a miniaturized scale have gained increasing interest \cite{waheed20163d}. These devices offer a multitude of advantages, like high throughput and efficiency, low production cost, low power consumption, parallel processing of samples, and fast sampling times. They are characterized by device geometries that exhibit extremely skewed aspect ratios (for instance, $1\times64\times 1024$), and with multiple objects within the device \cite{boy2008simulation}. This make octrees an attractive choice to simulate such devices. However, the skewed channel dimensions make it hard to deploy traditional octree approaches. Further, the presence of objects, such as sphere or pillar (to enhance the pressure drop, thus increasing the throughput ~\cite{zhao2017high} or get the desired focusing pattern ~\cite{kommajosula2019high,liu2017high,stoecklein2016optimization}) makes it even harder to mesh and simulate these devices.

\subsubsection{Simulation of Covid transmisson in classroom}
The COVID-19 pandemic has wreaked havoc on educational institutions. Best practice guidelines for safe in-person teaching is critical to ensure safe learning. In this context, high fidelity fluid simulations are a practical approach to evaluate various seating and operating scenarios~\citep{covid2020operating,wu2020effects}, identify risk factors, and rank order mitigation strategies. The availability of a fast mesh generation tool that can efficiently account for complex objects can significantly enable decision making by providing workflows that are rapidly deployable, personalized to specific room/scenario, and easy to extract reliable best practices.

%Most current simulation strategies utilize simplified assumptions for modeling the flow and aerosol distribution. We have exciting preliminary work that integrates four sophisticated concepts to provide very detailed estimates of aerosol distribution in indoor environments: (a) a detailed flow physics simulation (called Large Eddy Simulations) that produces significantly more accurate results while taking reasonable compute time, (b) accounting for the thermal plumes created by heat released by humans and electronics (which changes the flow in rooms), (c) immersogeometric analysis (see figures attached) that allows rapid exploration of a diverse array of configurations with complex geometries, (d) a detailed microdroplet distribution model that accounts for the distribution of droplet size due to evaporation, coalescence and breakup. There has not been any such high fidelity simulations performed to our best knowledge. 

%After the Covid pandemic hit United States in the March of 2020, the schools and colleges shut down. Many of the colleges did open in Fall for in-person classes, but some of them had to later shut down due to spike in the number of Covid cases. It remains an open question to how to safely open the colleges for in--person classes. The transmission of coronavirus in a classroom can be affected by a variety of factors like the sitting arrangements between the students in the classroom, the ventilation of the classroom or the humidity level ~\citep{covid2020operating,wu2020effects}. T

==> OldFiles/Dendro4Comparison.tex <==
Here, we compare the performance of the proposed algorithm with the existing octree based framework, specifically~\Dendro{}~ \cite{sampath2008dendro,sundar2008bottom,milinda_shayamal_fernando_2020_3876881}. \Dendro~ is a well-validated software and has been widely used in various large scale scientific simulations \cite{mukherjee2010performance,khanwale2020fully,saurabh2020industrial,fernando2018massively,xu2021octree,neilsen2018massively,neilsen2019dendro} and has over 200 citations. \Dendro~ has additional support for carrying out carving operations \cite{xu2021octree}. We choose \Dendro~ as our benchmark for comparison.  For comparison, we choose an elongated channel of dimensions $128 \times 4 \times 1$. The overall mesh is determined by two levels of refinement: base refinement and boundary refinement. Such a channel is commonly found in microfluidic devices, and simulating such devices is an active area of research~\cite{chai2011numerical,shen2004examination}. 

\input{Data/comparDendro4Table}
Table~\ref{tab:comparDendro4} compares the time for mesh generation and total \mvec{} time\footnote{This time include top-down, bottom up, leaf ~\mvec~ and ghost exchange time} for Navier--Stokes equation. Unlike the 3D Poisson operator used for scaling case, the time to compute elemental operator (denoted by leaf \mvec) is substantially more expensive. The extra overhead introduced by performing top-down and bottom-up traversal  will be significantly smaller compared to performing elemental ~\mvec. The overall time to solve is dominated by load balancing of FEM computation. Since ~\Dendro~ looks at the complete octree, a significant portion of the elements lie inside the void regions. The partitioning algorithm distributes the elements of complete octree (almost) equally among processors. This leads to an imbalance in the overall FEM computation. This is clear from the presented \mvec~ results. Additionally, in all our runs, we were not able to go beyond the level of 12 with the ~\Dendro~ framework. This limits our ability to compare for a further elongated channel. In contrast, within the current framework, we achieve a significant improvement in terms of both scalability and time to solve. \added{Overall, we observed a speedup of about 20$\times$ for mesh generation and 5$\times$ for \mvec~ time. The actual speedup that we can achieve is application-specific and needs to be studied individually. The major factors that determine the overall speedup can be mainly categorized as a) the fraction of volume that can be excluded out; b) complexity of \In--\Out test; c) the resultant communication pattern. }

==> OldFiles/DragCrisis.tex <==
\subsection{Validation case: Simulating drag crisis for flow past a sphere}\label{sec: DragCrisis}

% \input{Plots/SphereDrag}
\input{Plots/DragCombined}
We validate our numerical setup for Navier--Stokes simulation by computing the non-dimensional drag coefficient $C_d$ on sphere across a range of Reynolds number from 1 to 2,000,000. A sphere of diameter $d=1$ is placed at a distance $3d$ from the inlet at $(3d, \,3d,\, 3d)$ in a computation domain of $(10d, \,6d,\, 6d)$. The walls of the domain, except the outlet have constant non-dimensional freestream velocity of $(1, \, 0, \, 0)$ and zero pressure gradient. At the outlet, the pressure is set to 0 and zero gradient velocity boundary condition is applied at the wall. The no-slip boundary condition (zero Dirichlet) for velocity is imposed on the surface of sphere. The mesh resolution for the octree is varied depending on the Reynolds number and according to the Taylor's micro length scale. 
% In order to capture the curvature of the sphere accurately, the refinement level near the sphere was not dropped below 12 (\figref{fig: ProjectedArea}). 
Equivalently depending on the Reynolds number, the mesh in the wake region was refined to capture the turbulent structures. The spatial domain was discretized using linear basis function and the Crank Nicholson scheme was used for temporal discretization. 



\figref{fig: Drag} shows the variation of $C_d$ across the range of Reynolds number. We see that the results are in excellent agreement with the experimental result. It must be noted that we are able to accurately capture the drag crisis phenomena, where a sudden drop in drag from 0.5~\citep{achenbach1972experiments} - 0.6~\citep{bakic2003experimental} at Re around $16,000$ to 0.1~\citep{achenbach1972experiments} - 0.2~\citep{geier2017parametrization} at $Re$ of 2 million is observed. \added{~\figref{fig: SphereDragHighRe} shows the variation of $C_d$ with $Re$ on semi-log axis close to the drag crisis regime and compares with other numerical and experimental results from literature. We can see that our numerical results are in good agreement. Our finest resolution consists of around 40M elements which is close to the medium resolution for LBM simulation as done by ~\citet{geier2017parametrization}. No finer resolution is needed (or considered due to the high computational cost).} 

The prediction of drag crisis is of significant interest to the CFD community, with important engineering implications in aerodynamics and vehicular dynamics. We emphasize that no special numerical/modelling treatment is needed in this framework to capture the drag crisis; this is in contrast to existing work where typically a wall treatment~\citep{hoffman2006simulation,constantinescu2004numerical} is required to predict the drag crisis.


\figref{fig: wake} shows the turbulent flow structures with increasing $Re$. At $Re = 10,000$, the boundary layer becomes turbulent \figref{fig: Re10K}. With increase in $Re$, the vortices becomes smaller but the separation angle is not affected ($Re=160,000$ \figref{fig: Re160K}) until the critical regime is reached. \figref{fig: wake} gives the phenomenological description of drag crisis, which is evident by noticing the wake structure between \figref{fig: Re160K} at $Re=160K$ (subcritical regime) and \figref{fig: Re2M} at $Re=2\times 10^6$ (supercritical regime). In the subcritical regime, the wake behind the sphere tends to diverge as it moves away from the sphere. Above the critical $Re$, the wake tends to converge and become narrower as it moves behind the sphere. Subsequently, we can observe a high pressure zone being developed behind the sphere. The main reason for the drag crisis can be attributed to the development of this high pressure zone behind the sphere that tends to push the sphere in the inflow direction. These results are in agreement with the simulations by~\citet{geier2017parametrization} using Lattice Boltzmann method to capture the drag crisis.

\input{Plots/sphereDragLinear}


==> OldFiles/Results.tex <==

% \input{Plots/DragCrisis} 

% The overall thrust of this work is motivated by applications that require adaptive octrees for discretizing domains such as long channels or complex geometries. In such cases, the traditional method of generating octree fails on account of their symmetric nature in all the dimensions. These canonical applications exemplify the difficulty of anisotropic geometries as well as presence of multiple complex objects in the simulation domain. In this section, we present results for the target application. For all these simulations, we use well established Variational Multiscale (VMS) stabilized Finite Element method for solving Navier--Stokes equation~\citep{bazilevs2007variational}. \added{The solver has been validated by simulating the flow over sphere and has been shown to successfully capture the drag crisis. Please refer to \secref{sec: DragCrisis} for the validation case.}

% We begin by validating our framework using a canonical problem of flow past a sphere across a wide range of Reynolds numbers, encompassing the laminar-transition-turbulent regimes encompassing the drag crisis regime (\secref{sec: DragCrisis}). We then use our framework to estimate the enhanced pressure drop as a result of packing spheres in a microfluidic biosensing devices. (\secref{sec: microfluidics}). Finally, we deploy it to assess the impact of a specific seating arrangement on COVID-19 transmission-risk in a classroom.







% \figref{fig: wake} shows the turbulent flow structures with increasing $Re$.
% At $Re = 10,000$, the boundary layer becomes turbulent \figref{fig: Re10K}. With increase in $Re$, the vortices becomes smaller but the separation angle is not affected ($Re=160,000$ \figref{fig: Re160K}) until the critical regime is reached. \figref{fig: wake} gives the phenomenological description of drag crisis, which is evident by noticing the wake structure between \figref{fig: Re160K} at $Re=160K$ (subcritical regime) and \figref{fig: Re2M} at $Re=2\times 10^6$ (supercritical regime). In the subcritical regime, the wake behind the sphere tends to diverge as it moves away from the sphere. Above the critical $Re$, the wake tends to converge and become narrower as it moves behind the sphere. Subsequently, we can observe a high pressure zone being developed behind the sphere. The main reason for the drag crisis can be attributed to the development of this high pressure zone behind the sphere that tends to push the sphere in the inflow direction. These results are in agreement with the simulations by~\citet{geier2017parametrization} using Lattice Boltzmann method to capture the drag crisis.

% \begin{remark}
% It is worth noticing the difference in mesh resolution using immersed approach (IMGA) and \textit{carved} out approach. At low $Re$, the mesh resolution using the carved out is significantly higher than IMGA due to the fact that there is a minimum resolution needed to accurately capture the curvature of the sphere. But at high $Re$, the resolution required is mainly dictated by the boundary layer thickness, which dominates the resolution required to accurately capture the geometric curvature. IMGA, on the other hand suffer from the additional overhead of the surface discretization which should match the resolution of the background mesh. This makes the current framework a very promising tool to study high Reynolds flow.
% \end{remark}

% \input{Plots/MicrofluidPackedBed}

% \subsection{Microfluidic Biosensing Device} \label{sec: microfluidics}

% \input{Plots/packedBedSetup}

% \figref{fig:packedBed} shows the simulation setup for a microfluidic biosensing device. The applied electric current through the device creates ion concentration depletion as well as a high electric field near the array of spheres. The target analytes, such as DNA or virus are accumulated in this high electric field region, which enhances the sensitivity of the microfluidic biosensor. The mechanism of the proposed device encompasses multi-physics including mass transport, electrodynamics, and fluid physics. Navier-Stokes coupled with Poisson-Nernst-Planck (NS-PNP) is used to simulate these types of behaviour. A key first metric of interest is to evaluate the pressure drop across the packed bed, which can be computed by solving the Navier-Stokes equation and measuring the pressure drop. The pressure drop plays an important role in determining the manufacturability of these microfluidic devices. A high pressure drop is needed for high throughput, but an excessive pressure drop can collapse the microchannel. These simulations provide a preliminary check and allows for the estimation of device failure conditions based on various design parameters.

% The computation domain is a channel of dimensions $16 \times 1 \times 128$. A packed bed consisting of 10 layers array of spheres packed in a BCC (body centered cubic) pattern is placed in the interior of the channel. We carve out each individual sphere in this packed bed from the background mesh. The inlet velocity of $(1, \, 0, \, 0)$ is applied at the inlet. The no-slip velocity is applied on all the walls and spheres in the packed bed. A zero gradient pressure boundary condition is applied on the walls and sphere boundaries except at outlet, where a zero Dirichlet pressure is set. 

% \figref{fig:micro-channelVelocity} shows the flow pattern around the packed bed of spheres. As the flow reaches the packed bed it accelerates and passes through the void region around the spheres. \figref{fig:pressureDrop} compares the pressure drop due to the presence and absence of the packed bed. In the absence of the packed bed of spheres, the pressure drop follows a linear profile with high pressure at the inlet and low pressure at the outlet, which is characteristic of channel flow. The presence of the packed bed of sphere leads to sharp increase in pressure drop near the region of sphere packing. Away from the packing region, the pressure drop again follows the linear profile. Overall, the packing of sphere increases the pressure drop in the micro channel.

% \begin{remark} We emphasize that this simulation was possible only with the traversal-based matvec approach. The traditional approach using neighborhood data structures fails to simulate such an elongated micro-channel on account of isotropic nature of octrees. The presence of such closely packed spheres make it hard even for unstructured grid to mesh these domain, whilst maintaining the aspect ratio. The proposed traversal-based approach provides a robust way to adaptively refine the region of interest based on a series of \In - \Out tests.
% \end{remark}


\subsubsection*{\textbf{Validation}:\;} We first validate the solver by demonstrating the ability to capture the drag crisis by simulating flow past a sphere. A sphere of diameter $d=1$ is placed at a distance $3d$ from the inlet at $(3d, \,3d,\, 3d)$ in a computation domain of $(10d, \,6d,\, 6d)$.  The walls of the domain, except the outlet have constant non-dimensional freestream velocity of $(1, \, 0, \, 0)$ and zero pressure gradient. At the outlet, the pressure is set to 0 and zero gradient velocity boundary condition is applied at the wall. No-slip boundary condition (zero Dirichlet) for velocity is imposed on the surface of the sphere. We use a well-established Variational Multiscale (VMS) stabilized Finite Element method for solving the Navier--Stokes equation~\citep{bazilevs2007variational}.

~\figref{fig: DragSemiLinear} plots the variation of $C_d$ across a range of Reynolds numbers close to the drag crisis regime. We see that the results are in excellent agreement with experimental and other numerical results.  We are able to accurately capture the drag crisis phenomena, where a sudden drop in drag from 0.5~\citep{achenbach1972experiments} - 0.6~\citep{bakic2003experimental} at Re around $16,000$ to 0.1~\citep{achenbach1972experiments} - 0.2~\citep{geier2017parametrization} at $Re$ of 2 million is observed. The finest resolution simulation consists of $\sim$40M elements which is significantly lower than for LBM simulation by ~\citet{geier2017parametrization}. We visualize the transition across the drag crises regime in ~\figref{fig: wake}. The drop in drag in ~\figref{fig: DragSemiLinear} is due to the change in wake structure and pressure distribution in ~\figref{fig: wake}.
\begin{figure}[t!]
    \centering
    \includegraphics[trim=0 90 0 100, clip,width=0.99\linewidth]{Images/classroomDomain.pdf}
    \caption{Figure showing the classroom domain and different regions of boundary conditions such as velocity inlet and pressure outlet. The right side shows the zoomed image with mesh refinement near the object. In all our simulations, we consider that the person marked in red is COVID positive.\vspace{2 mm}}
    \label{fig:classroomDomain}
\end{figure}

\input{Plots/classroom}
\textbf{Application}: We finally demonstrate the ability of our framework to simulate flow past complex geometries. We consider a realistic scenario of modeling airflow in a classroom with complex furniture, seated students with/without computers (and monitors), and a standing instructor. \added{We are particularly interested in accessing if specific locations in the room are at significantly higher risk for transmission -- for example, where there is local recirculation causing limited air exchange with the outside environment. In such cases, it becomes imperative to identify if such locations have a higher risk and rank among alternate seating arrangements to mitigate this risk. The current incomplete octree framework allows us to efficiently and rapidly evaluate various seating arrangements and scenarios. %We solve the Navier-Stokes equations for realistic air exchange rates for two cases, and subsequently simulate scalar transport of aerosolized viral particles (modeling a cough from a infected individual).
% (see Fig.~\ref{fig:test}).
} In order to \textit{carve} out the geometry, we perform a series of \In - \Out tests. This gives an automated way to carve out complex geometries from the domain. \figref{fig:classroomDomain} shows the computational domain of size  $4.83 \times 3.34 \times 1$ that includes complex features such as tables, chairs and mannequins representing students and instructor. The velocity inlets and pressure outlets are located at the top of the domain.  The non-dimensional inlet velocity of $(0, 0, -1)$ is imposed at velocity inlets and zero pressure at pressure outlets. $Re = 10^5$ was considered based on the inlet velocity and classroom height. These flow rates, air exchange rates, and room geometry represent typical values in classrooms seen in US schools.
% \added{\figref{fig: COVIDClassroom_1} shows the computational domain that includes complex features such as tables, chairs, and mannequins representing students and instructors. Four velocity inlets are located at the top of the domain, and four pressure outlets are at the front and back of the domain. The computational domain is $4.83 \times 3.34 \times 1$; the non-dimensional inlet velocity is $(0, 0, -1)$ at four rectangular regions on the top of the domain, zero pressure outlet on the side of the domain, the remaining boundaries are no-slip velocity boundary. $Re = 10^5$ based on the inlet velocity and classroom height. These flow rates and room geometry represent typical values seen in US universities.}

\added{Fig.~\ref{fig:test} illustrates preliminary results enabled by our framework to evaluate the transmission of COVID viral load in the classroom. We evaluate the impact of one infected individual (colored red) who periodically coughs, releasing an aerosolized load of viral particles. We model the time-dependent transmission of the viral load as a scalar transport equation that is advected by a statistically steady--state flow field obtained from the solution of Navier--Stokes solver. We considered a classroom under two different scenarios: with (\figref{fig:classroom:Monitors}) and without (\figref{fig:classroom:noMonitors}) the presence of computer monitors. We observe a significant reduction in transmission risk in the case with monitors due to the monitors redirecting the flow field upwards away from the occupied zone.}
\input{Data/ibmComparD5}
\input{Data/tabScalingClassroom}

\added{\tabref{tab:comparD5} compares the IMGA based immersed implementation (based on the open-source code~\cite{Dendrite})  with the carved-out approach. The overall mesh consists of three refinement levels: base refinement, exit refinement (near the velocity inlet and pressure outlet), and object refinement (near the monitors, tables, and mannequin). To get the refined final mesh, we start the mesh at the base level and successively refine the mesh until the required refinement level is reached. At each iteration, we perform a series of ray-tracing to determine~\In or \Out relative to the object. Overall, we see an approximately 50\% increase in element size for the immersed case.  We achieve a speedup of approximately 2.2$\times$ during the mesh creation stage and 2.8$\times$ for the complete solve time. The speedup obtained in this case is significantly smaller than the channel case described in \secref{sec: comparD4} mainly because of the nature of objects being carved out. The mannequin or the table considered here has a large surface area to volume ratio. The small volume resulted in most of the octants percolating close to the finest level before they can be discarded. Additionally, ray-tracing based \In-\Out test needs to be performed at each iteration of refinement, which is quite expensive \cite{saurabh2020industrial}. Once the mesh is generated, we see a significant speedup in the overall solve time. \tabref{tab:scalClassroom} compares the scaling efficiency for two different meshes. Overall we achieve a good scaling efficiency of about 90\% over 16 fold increase in the number of processors.}
%Please refer to the \secref{appendix:classroom} for additional details on the computational domain. Using this computational domain, we can compute the probability of the airflow reaching other students from one student.






% \added{\figref{fig: COVIDClassroom_2} shows the flow-field structure of the middle plane, as well as streamlines, originated from points around the head region of a student. The line integral convolution plot shows the re-circulation region is separated between students. The streamlines show that the increased distance between students decreases airflow from one student reaching another student.}

% \begin{figure}
%     \includegraphics[width=0.99\linewidth]{Images/COVID-Classroom-1.png}
%     \caption{Figure showing the computational domain, boundary condition and enlarged mesh slice for the classroom simulation. The computation domain consists of a cuboid domain of $4.86 \times 3.34 \times 1 $, with six sets of tables, chairs and sitting mannequins as well as one standing mannequin represented by STL files.}
%     \label{fig: COVIDClassroom_1}
% \end{figure}

% \begin{figure}
%     \includegraphics[width=0.99\linewidth, trim=70 0 80 0, clip]{Images/COVID-Classroom-2.png}
%     \caption{Figure showing one vertical slice of line integral convolution plot around the middle plane of the classroom and streamlines from around the head region of one student}
%     \label{fig: COVIDClassroom_2}
% \end{figure}

% Moved to appendix
%\input{Plots/COVIDClassroom}

%\figref{fig: COVIDClassroom_1} shows the computational domain that includes complex features such as tables, chairs and mannequins representing students and instructor. Four velocity inlets located at the top of the domain and four pressure outlets are at the front and back of the domain. The computational domain is $4.83 \times 3.34 \times 1$, the non-dimensional inlet velocity is $(0, 0, -1)$ at four rectangular region on the top of the domain, zero pressure outlet on the side of the domain, the remaining boundaries are no-slip velocity boundary. $Re = 10^5$ based on the inlet velocity and classroom height. This flow rates and room geometry represent typical values seen in US universities. 


%\figref{fig: COVIDClassroom_2} shows the flow-field structure of the middle plane, as well as streamlines originated from points around the head region of a student. The line integral convolution plot shows the re-circulation region is separated between students and the streamlines shows the increase distance between students decrease the chance of airflow from one student reaching other students. 

% \begin{remark}
% The framework allows us to carve out the complex geometries and perform simulations while retaining small geometric features. This remains difficult for traditional body-fitted mesh approaches, especially when we seek to explore various seating scenarios. 
% \end{remark}

==> OldFiles/ad.tex <==
% artifact description goes here. 
% \appendix
% \subsection{Artifact Availability}
\subsection{Libraries dependencies}
The following dependencies are required to compile the code:
\begin{itemize}
	\item C/C++ compilers with C++11 standards and OpenMP support
	\item MPI implementation (e.g. openmpi, mvapich2 )
	\item \petsc~ 3.8 or higher
	\item ZLib compression library (used to write \texttt{.vtu} files in binary format with compression enabled)
	\item  MKL / LAPACK library
	\item CMake 2.8 or higher version
	\item \href{http://hyperrealm.github.io/libconfig}{libconfig} for parameter reading from file.
\end{itemize}


\subsection{\Frontera~ environment}
Experiments performed in \Frontera~ are executed in the following module environment. 
\begin{verbatim}
Currently Loaded Modulefiles:
  1) intel/19.0.5   4) python3/3.7.0
  2) impi/19.0.5    5) autotools/1.2
  3) petsc/3.12     6) cmake/3.16.1
\end{verbatim}

\subsection{\Frontera~ compute node configuration} \label{sec:Frontera}
\begin{verbatim}
    Architecture:          x86_64
    CPU op-mode(s):        32-bit, 64-bit
    Byte Order:            Little Endian
    CPU(s):                56
    On-line CPU(s) list:   0-55
    Thread(s) per core:    1
    Core(s) per socket:    28
    Socket(s):             2
    NUMA node(s):          2
    Vendor ID:             GenuineIntel
    CPU family:            6
    Model:                 85
    Model name:            Intel(R) Xeon
                           Platinum 8280
                           CPU @ 2.70GHz
    Stepping:              7
    CPU MHz:               2700.000
    BogoMIPS:              5400.00
    Virtualization:        VT-x
    L1d cache:             32K
    L1i cache:             32K
    L2 cache:              1024K
    L3 cache:              39424K
    
    MemTotal:       195920208 kB
    MemFree:        168962328 kB
    MemAvailable:   168337408 kB
\end{verbatim}



==> OldFiles/ae.tex <==
\subsection{Signed distance computation}
\input{signedDistance}
\subsection{Details of solver selection}
\petsc~ was used to solve all the linear algebra problems. In particular, bi-conjugate gradient descent (\texttt{-ksp\_type bcgs}) solver was used in conjunction with Additive - Schwartz (\texttt{-pc\_type asm}) preconditioner to solve the linear system of equations. The \textsc{NEWTONLS} class by \petsc, that implements a Newton Line Search method, was used for the nonlinear problems. Both the relative residual tolerance and the absolute residual tolerance for linear and non - linear solve are set to $10^{-6}$ in all numerical results.

% \input{Plots/DragCrisis}
% \input{DragCrisis}

% \input{classroomAE}





% \subsection{Classroom simulations}\label{appendix:classroom}

% \input{Plots/COVIDClassroom}

% \figref{fig: COVIDClassroom_1} shows the computational domain that includes complex features such as tables, chairs and mannequins representing students and instructor. Four velocity inlets located at the top of the domain and four pressure outlets are at the front and back of the domain. The computational domain is $4.83 \times 3.34 \times 1$, the non-dimensional inlet velocity is $(0, 0, -1)$ at four rectangular region on the top of the domain, zero pressure outlet on the side of the domain, the remaining boundaries are no-slip velocity boundary. $Re = 10^5$ based on the inlet velocity and classroom height. This flow rates and room geometry represent typical values seen in US universities. 


% \figref{fig: COVIDClassroom_2} shows the flow-field structure of the middle plane, as well as streamlines originated from points around the head region of a student. The line integral convolution plot shows the re-circulation region is separated between students and the streamlines shows the increase distance between students decrease the chance of airflow from one student reaching other students. 

\subsection{Downloading and installing the code}
This section presents how to run and reproduce the results presented in the paper. You can clone the repository using, \texttt{git clone https://bitbucket.org/baskargroup/sc21-kt.git}

(DOI: 10.5281/zenodo.5168313). 

We use \texttt{CMake} to configure and build. In \Frontera~node, 
\begin{itemize}
    \item \texttt{git clone https://bitbucket.org/baskargroup/sc21-kt.git}
    \item \texttt{mkdir build \&\& cd build}
    \item Load the module environment
    \item \texttt{mkdir build \&\& cd build}
    \item \texttt{cmake ../.}
    \item \texttt{make MVCChannel MVCSphere signedDistance}
\end{itemize}

\subsection{Running experiments}
\subsubsection{\texttt{MVCChannel}: \;} Scaling  run for channel case. In order to run the scaling case, it requires the 3 parameters: a) baseLevel b) boundaryLevel and c) element order (1/2). For example, on ~\Frontera~ it can be ran as:

\texttt{ibrun MVCChannel 10 12 1 log10\_12.out} 

\noindent where, 10 is the base refinement level, 12 is the boundary refinement level, 1 is the element order and \texttt{log10\_12.out} is the output file containing the relevant timing information.

\subsubsection{\texttt{MVCSphere}: \;}
Scaling  run for sphere case. In order to run the scaling case, it requires the 3 parameters: a) baseLevel b) boundaryLevel and c) element order (1/2). For example, on ~\Frontera~ it can be ran as:

\texttt{ibrun MVCSphere 7 12 1 log7\_12.out} 

\noindent where, 7 is the base refinement level, 12 is the boundary refinement level, 1 is the element order and \texttt{log7\_12.out} is the output file containing the relevant timing information.

\subsubsection{\texttt{signedDistance}: \;} The computation of signedDistance. In order to find the signed distance, we successively refined near the boundaries and computed the signed distance. In order to run the code:

\texttt{ibrun signedDistance stlFileName 4 14}

\noindent where: \texttt{stlFileName} is the name of stl file, 4 is the minimum refinement level and 14 is the maximum level of refinement at the stl boundary. After each successive iteration, the code output the information of boundary nodes. Then we compute the signed distance, using the python script provided under the \texttt{scripts} folder. In order the run the python scripts:

\texttt{python3 signedDistance stlFileName}.


Note that you might need to change the number of processor on your machine as the python script is parallel and make use of \texttt{multiprocessing} library.


\subsubsection{Roofline plot: \:}

We computed the roofline using Intel Advisor. In order to run the roofline plot, first run the survey using:

\noindent\texttt{ibrun -np 1 advixe-cl -collect survey -project-dir outputDir
           -search-dir \\
           src:=examples/BenchMark\_channel/src 
           -- MVCChannel \\
           baseLevel boundaryLevel eleOrder outputFile}
           
\noindent where: 
\text{outputDir} is the directory to store output and \texttt{MVCChannel   baseLevel boundaryLevel eleOrder outputFile} is the same as in previous description of Channel scaling.

Finally in order to collect FLOPS count:

\noindent\texttt{ibrun -np 1 advixe-cl -collect=tripcounts
           --flop  \\
            --mark-up-list= src/benchmark.cpp 
            -project-dir= outputDir 
            -- MVCChannel baseLevel \\
            boundaryLevel eleOrder outputFile}
            
\noindent where:
\text{outputDir} must be same directory as the survey directory and \texttt{MVCChannel} must be called with the same arguments.

==> OldFiles/classroomAE.tex <==
\subsection{Classroom Simulation: Computational Domain and Boundary Conditions}
\label{sec:classroomAE}

\figref{fig:classroomDomain} shows the computational domain that includes complex features such as tables, chairs and mannequins representing students and instructor. The velocity inlets and pressure outlets are located at the top of the domain. 
\subsubsection{Navier--Stokes simulation:\;}
The computational domain is $4.83 \times 3.34 \times 1$, the non-dimensional inlet velocity is $(0, 0, -1)$ at velocity inlets and zero pressure outlet on the side of the domain. the remaining boundaries are no-slip velocity boundary. $Re = 10^5$ based on the inlet velocity and classroom height. This flow rates and room geometry represent typical values in classrooms seen in US schools and universities. 

\subsubsection{Advection--Diffusion equation:\;} Once an statitstically stationary state has been achieved, we use the averaged velocity field to solve the advection--diffusion equation (scalar transport).  The initial cough releases viral particles in a conical region near the mouth of the mannequin and is evolved using the advection diffusion equations.


==> OldFiles/condition.tex <==
% \input{Plots/Condition}
As stated earlier, one approach to deploy traditional octrees on elongated channels is to stretch the mesh along the elongated channel ~\cite{esmaily2018scalable,mani2012analysis}. But this has a detrimental effect on condition number, which in turn will deteriorate the convergence of linear solvers. Table~\ref{table: conditionNumber} compares the variation in the condition number \footnote{evaluated with Matlab \texttt{condest} command} with the stretching of the elements for a  Laplace operator in 2D. We can see that with the increase in the aspect ratio of the mesh, the condition number of the linear system increases. With the generation of incomplete octree, we can ensure the aspect ratio of  each element in the mesh remains 1. Furthermore, since the error is dominated by the coarsest resolution, the incomplete octree permits decreasing the overall DOFs, at a given coarse resolution. This, in turn, decreases the condition number of the linear system.
\input{Data/tableConditionNumber}


==> OldFiles/convergence.tex <==
 Here, we present the convergence analysis for the Poisson operator $- \Delta u = f$ over the domain $\Omega$ with $u  = u_D$ on the domain boundary $\Gamma$. Inserting appropriate finite dimensional function spaces for trial and test function, the weak form of the Poisson operator can be written as: $(\nabla w^h,\nabla u^h)_{\Omega} = (w^h,f)_{\Omega}$
\begin{equation}
    (\nabla w^h,\nabla u^h)_{\Omega} = (w^h,f)_{\Omega}
\end{equation}

As mentioned previously, deploying incomplete octree based methods results in a voxelated geometry for a complicated geometrical shape. As discussed in~\secref{sec: signeddistance}, with the increase in the refinement of the element, the voxelated geometry approaches the true geometry. The rate of convergence of the distance follows only first order. Therefore, careful treatment is needed at the boundary elements to ensure an accurate order of convergence. In this context, several methods have been proposed in the literature~\cite{mittal2005immersed,lee2013implicit,burman2012fictitious}. In this work, we use the Shifted Boundary Method (SBM)~\cite{main2018shifted,atallah2020second} to treat boundary elements. 

The main idea behind SBM is to reformulate the original boundary value problem over a surrogate computational domain by modifying the original boundary conditions using Taylor series expansions. The weak form of Poisson operator after applying SBM treatment can be written as:
\begin{equation*}
\begin{split}
    (\nabla w^h, \nabla u^h)_{\Tilde{\Omega}} - (w^h,\nabla u^h \cdot \Tilde{\mathbf{n}})_{\Tilde{\Gamma}} - (\nabla w^h \cdot \Tilde{\mathbf{n}}, u^h + \nabla u^h \cdot \mathbf{d} -u_D)_{\Tilde{\Gamma}} + \\
    \frac{\alpha}{h}(w^h + \nabla w^h \cdot \mathbf{d}, u^h + \nabla u^h \cdot \mathbf{d} - u_D)_{\Tilde{\Gamma}} = (w^h,f)_{\Tilde{\Omega}}
\end{split}
\end{equation*}
where $\Tilde{\Omega}$ is the voxelated domain, $\Tilde{\Gamma}$ is the surface of the voxelated domain, $\Tilde{n}$ is the unit normal of the voxelated surface, $\alpha$ is the penalty term, $h$ is the element length, and $\textbf{d}$ is the distance vector from the boundary surface of voxelated domain $\Tilde{\Gamma}$ to the true surface $\Gamma$. The main idea of the method is to shift the boundary condition from $\Gamma$ to $\Tilde{\Gamma}$ by using second-order accurate Taylor series expansion. We omit the details here and refer to~\cite{main2018shifted,atallah2020second} for detailed analysis.

To perform the convergence study, we consider Poisson problem on a two-dimensional disk of radius $R = 0.5$, centered at $(x_0 = 0.5,y_0 = 0.5)$ and $f = 1$. An exact solution exists and can be written as:
\begin{equation}
    u(r) = 0.25(R^2 - r^2)
\end{equation}
where $r = \sqrt{(x-x_0)^2+(y - y_0)^2}$.~\figref{fig:convergence} shows the convergence behaviour for the linear basis function. If we naively apply the boundary condition at the boundary nodes of the voxelated geometry, we only get a first-order convergence in both $L_2$ and $L_\infty$ norm. This is because the right boundary condition is applied at the wrong place, which is shifted by a distance $\mathbf{d}$ from the true boundary. As seen from the signed distance plot (\figref{fig:DragonError}), the voxelated geometry boundary approaches the true geometry according to the first order, and so is the convergence for the discrete Poisson operator. With the SBM method, we recover back the theoretical second-order convergence in both $L_2$ and $L_\infty$ norm for the linear basis function.

\input{Plots/convergence}


==> OldFiles/dofTest.tex <==
Here, we present the comparison of the carved out approach with the immersed approach in terms of the  number of DOF and the total number of elements. We note that this analysis is equation agnostic. In order to compare the overall mesh element size and DOF, we set the background mesh to a constant refinement level and refined it near the object. \tabref{tab:dofCompar} compares the fraction of elements and DOF required for immersed and carved out approach. In the carved out case, all the elements and nodes that are inside the domain are discarded during the tree construction as mentioned in \secref{sec: octreeConstruct}, whereas for the immersed case, we retain the complete octree mesh. 2:1 balancing of octrees leads to the ripple effect, because of which there is a significant number of elements that are inside the domain (\figref{fig: meshComparison}). The nodes and elements that are marked \In (i.e. inside the object, sphere/dragon in this case) do not contribute towards the accuracy of the solution. These are not solved for in the system of equations, and eventually, a Dirichlet boundary condition is applied to it, but they had the associated cost during tree traversal and memory footprint for matrix and vector storage. \added{Overall, we see about an increase of 80--90\% in element size and a 33--40\% in the DOF count if we immerse an object.} The excess DOF count is significantly smaller than the element count because of the fact that we are performing continuous Galerkin (CG) computations and several elements share a common DOF. Additionally, we must recall the fact that in CG computations, hanging nodes do not contribute to the additional degrees of freedom. However, if we were to perform discontinuous Galerkin (DG) computation, each element would have its own unique node id and associated DOF. In such computations, the excess DOF count would scale as excess element count. The actual fraction of DOF and element that is reduced as a result of carving out depends upon the surface area and volume of the object that is being carved out. \added{A large surface area of the object would result in more elements at the finest resolution near the boundaries of the object. In contrast, a larger volume would result in more elements being discarded out from the interior of the object.} Constructing an incomplete octree by cutting the elements inside the object results in processing fewer elements during a solve. 
% \input{Plots/ComparisonElements}
\input{Data/tabDofCompar}


==> OldFiles/introduction.tex <==
% \begin{itemize}
%Partial differential equations (PDEs) are ubiquitous in nature and is used to model the phenomena ranging from fluid flow (Navier--Stokes), electromagnetism (Maxwell equation) to Quantum mechanics (Schrodinger equations). The solution to these PDEs holds the key to understand the various natural process from the atomic scale like the movement of electrons~\citep{pierret1987advanced} to the astronomical scale like clumping of galaxies in universe~\citep{tremaine2003origin}. The solution to these PDEs holds a key to understand and solve the pressing problem of the current century like climate change~\citep{muller2014massively}, weather forecasting~\citep{zjavka2014forecast}, water purification~\citep{queinnec2006development} or cancer treatment~\citep{amoddeo2015moving}. In real world application, due to the complexity of equation, boundary condition and the overall domain geometry, the analytical solution are not known, and hence the numerical solutions are needed to understand them. 

% Partial differential equations (PDEs) are ubiquitous and are used to model various natural phenomena. The ability to solve PDEs numerically is essential, especially for designing engineered systems. %Numerical solutions for PDEs hold the key to understanding the various natural processes from the atomic scale\citep{pierret1987advanced} to the astronomical scale\citep{tremaine2003origin}. 
% Solutions to these PDEs hold the key to understand and solve pressing problems of the current century, like climate change~\citep{muller2014massively}, weather forecasting~\citep{zjavka2014forecast}, and water purification~\citep{queinnec2006development}.% or cancer treatment~\citep{amoddeo2015moving}. 

%Meshes play a pivotal role in determining the quality and accuracy of solutions of these numerical methods. Although, such a fundamental and integral part of PDE solver, mesh generation, still continues to be a major bottleneck and time consuming process in the overall workflow. This becomes even more challenging in the presence of a complex object, wherein the stated object has to be \textit{carved} out from the domain in order to solve the PDE with the appropriate level of refinement. This problem has also been highlighted as one of the component of NASA CFD 2030 challenge towards the goal of conducting overnight LES~\citep{slotnick2014cfd} which states : \textit{Mesh generation and adaptivity continue to be significant bottlenecks in the CFD workflow..} 
The discretization of the domain (i.e., mesh generation) is a critical aspect of numerically solving PDEs. The resolution and quality of the mesh are intimately related to the overall accuracy of PDE solvers. Even though mesh generation is a fundamental part of numerical approaches, creating quality meshes continues to be a significant bottleneck in the overall workflow. This bottleneck is exacerbated when considering adaptivity and parallel deployment and becomes exceptionally challenging in the presence of an arbitrarily shaped geometric object that has to be \textit{carved} out from the computational domain. Such challenges are particularly common in simulating the flow over external objects. Streamlining this workflow is one of the components of the NASA 2030 computational fluid dynamics (CFD) milestone towards the goal of conducting overnight large-eddy simulations (LES)~\citep{slotnick2014cfd}: \textit{"Mesh generation and adaptivity continue to be significant bottlenecks in the CFD workflow."} 

%Immersed boundary (IBM) approaches has been looked as an alternative to alleviate these time consuming and laborious approaches, wherein the complex object is \textit{immersed} in the fluid domain. The major advantage of using the immersed approaches is to perform the complete simulation on a structured grid~\citep{peskin1977numerical, mittal2005immersed}, and thus avoids the requirement for the grid to conform to the complex shape. Unfortunately, this has also made the application of the kinematic boundary conditions such as no-slip on the surface of immersed boundaries non-trivial~\citep{kim2001immersed,saurabh2020industrial,tseng2003ghost}. In this work, we present a fast alternative approach to IBM, wherein the object is still \textit{carved} out from the tree based generated mesh. This retains the simplicity of the mesh generation approach provided by tree based data structure along with the advantages possessed by the body conforming grid.

Immersed boundary methods (IBMs)~\citep{mittal2005immersed} are commonly used to simulate fluid flow around geometric objects \textit{immersed} in a computational domain. A significant advantage of IBM approaches arises from performing the complete simulation on structured grids~\citep{peskin1977numerical, mittal2005immersed}, thus avoiding any requirement of the grid conforming to the immersed geometric object (\figref{fig:immersed}). 
%Unfortunately, this also makes the enforcement of the kinematic boundary conditions such as no-slip on the surface of immersed boundaries non-trivial. Over the past two decade, there has been a lot of work has been focused to analyze the impose the kinematic boundary condition accurately~\citep{kim2001immersed,saurabh2020industrial,tseng2003ghost}. 
Naively immersing the object can lead to large void regions. These regions do not participate in the solution but require the associated matrix and vector storage as they form a part of the mesh data structure. This problem is exacerbated in the presence of multiple objects. This paper presents a strategy wherein the void regions are first \textit{carved} out from the main computational domain (\figref{fig:carved}) ---in the vein of the finite cell approach~\citep{varduhn2016tetrahedral} with the object then immersed in the carved domain. This approach reduces the number of degrees of freedom and, hence, the memory footprint associated with the void regions.

% Such an approach retains the simplicity of the mesh generation provided by tree-based data structure along with the advantages of the simple imposition of boundary conditions afforded by a body-conforming grid (\figref{fig:carved}). 
% Figure \ref{fig:carvedFig} illustrates the difference in the mesh generated between an immersed versus a carved-out approach leading to the generation of complete and incomplete trees respectively.

\input{Plots/meshComparisonFigs}

Tree-based grid generation (quadtrees in 2D and octrees in 3D) is common in computational sciences \citep{tu2005scalable,ishii2019solving,fernando2018massively,sundar2008bottom,bastian2008generic,greaves1999hierarchical,bader2012space,BursteddeWilcoxGhattas11,popinet2003gerris} largely due to its simplicity and parallel scalability. The ability to efficiently refine (and coarsen) regions of interest using tree-based data structures have made it possible to deploy them on large-scale multi-physics simulations~\citep{akhtar2013boiling,saurabh2020industrial,fernando2018massively,khanwale2020fully,rudi2015extreme,bielak2005parallel,losasso2004simulating,kim2003large,agbaglah2011parallel,losasso2004simulating}. Existing algorithms for tree-based grid generation are mainly focused on axis-aligned hierarchical splitting on isotropic domains (i.e., spheres, squares, and cubes). Such approaches cannot easily support anisotropic domains (for example, an elongated channel) or body-conforming mesh generation for a carved-out object. Standard workarounds include stretching or warping (using a coordinate transformation) of the computational domain, transforming a cubic domain into a rectangular channel. Unfortunately, these asymmetric transformations come at the cost of degradation in the overall quality of the domain discretization leading to large condition numbers in the resultant matrix (see \secref{sec:ConditionNumber}).

% An alternate approach has been to use two-tier meshes \cite{hhg04,BursteddeWilcoxGhattas11} that rely on having a top-level unstructured hexahedral mesh that conforms to the complex geometry and can independently refine (uniformly or adaptively) each hexahedral element of the top-level mesh. While this approach works well for simple shapes, like spheres \cite{sc08-seismic}, hex-meshing is non-trivial for more complex geometries \cite{viertel2019approach}. An alternative is then to use affine transforms within each top-level element but limits the ability to have isoparametrically refined elements. In contrast, our approach can take an arbitrary function to carve out the domain and is capable of on-the-fly refinement and coarsening that matches the arbitrary function within the refinement tolerance.  


% The tree based data structure (quadtree in 2D and octree in 3D), on account of its conceptual simplicity and ability to scale across large number of processors, has been an attractive choice as a mesh generation tool for solving PDEs~\citep{tu2005scalable,ishii2019solving,fernando2018massively, sundar2008bottom}. The ability to refine and coarsen in the area of interest using these tree based data structure have made it possible to deploy them on large scale multiscale and multiphysics simulations.~\citep{saurabh2020industrial,fernando2018massively,khanwale2020fully,rudi2015extreme}

%\textbf{tries to compensate for the symmetric refinement nature of octrees}
 
%\textbf{elongated geometries - creates anisotropic elements}
  
% \textbf{complex geometries }
   
%\textbf{reducing the number of elements and dof
%   Conditioning of resulting operators}
% \mf{Add this}
%\textit{\sout{ Most of the literature have been focused on fast generation of these tree based data structure on an isotropic domain (cube / square). This is primarily due to their symmetric nature in all the dimension. In presence of elongated domain, one viable approach will be to stretch the elements along the elongated dimension, but this will affect the condition number of matrices and deteriorate the convergence of numerical solver. This becomes even more complicated in presence of complex generation. The presence of the complex geometries leads to the void regions resulting in an incomplete tree based data structure. }}

Our contributions in this paper are as follows: (a) we develop an efficient tree-based adaptive mesh generation framework that relaxes the requirement of the mesh to conform to isotropic domains; (b) we compare the current approach with the state-of-the-art \textit{immersed} method strategies~\citep{xu2016tetrahedral,kang2011comparative,wang2008combined,uhlmann2005immersed}; (c) we show the parallel scalability of our framework on the~\Frontera{} supercomputer up to 16K cores; (d) we deploy the framework in conjunction with a well established FEM formulation: variational multiscale (VMS) method~\citep{bazilevs2007variational} to model non-trivial applications of simulating the flow fields in classrooms to understand the risk of transmission of Coronavirus. The fast generation of quality meshes is pivotal to this application. Here, we present an octree-based mesh generation tool that provides an alternative to using two-tier meshes (HHG~\cite{hhg04}, p4est~\cite{BursteddeWilcoxGhattas11}) and is not dependent on having top-level hexahedral meshes--that can be hard to generate. In contrast, our approach works with any arbitrary user-supplied function that returns \In or \Out (of the object) for any queried point.

% Short on space
% The rest of the paper is organized as follows: we begin by introducing the definition of subdomain and key algorithmic developments for efficient mesh generation in \secref{sec: Methods}; we showcase the advantages of generating incomplete octrees and present scaling result in \secref{sec: Results}; we show the results of our target application in \secref{sec: ResultApplication} and finish by laying out our conclusion and future outlook in \secref{sec: Conclusion}. 

\section{Related Work}
\label{sec:related_work}
There have been significant algorithmic advances for the fast generation of octrees on modern supercomputers. For instance, octrees have been used for voxelization of 3D objects to accelerate ray-tracing~\citep{whang1995octree}, signed distance calculation~\citep{yu2015scalable}, compression~\citep{samet2002octree}, and fast rendering~\citep{laine2010efficient}. Building upon these successes, octrees have become one of the more common mesh generation tools for large-scale PDE simulations, with scalable and adaptive capabilities~\citep{tu2005scalable,egan428direct,rudi2015extreme,khanwale2020fully,fernando2018massively,griffith2007adaptive}.
But most work related to solving PDEs has been focused on the generation of \textit{complete} octrees in the context of PDE solvers \cite{sampath2008dendro,sundar2008bottom,fernando2017machine,fernando2018massively,ishii2019solving,weinzierl2019peano,macri2008octree,teunissen2018afivo,camata2013parallel}.
In a complete octree, every non-leaf subtree has all $2^d=8$ children,
and thus, the union of all leaf octants is a filled cube without holes. This makes simulating non-cuboid domains non-trivial, with most approaches either relying on stretching (coordinate transforms) or using a much larger bounding box.  Secondly, complex objects have to be \textit{immersed} into the octree mesh \cite{saurabh2020industrial,egan428direct,griffith2007adaptive}, rather than being \textit{carved-out}. Naively immersing the object in the octree can leave many elements that fall into the void regions. This problem is further exacerbated in the presence of multiple objects. The elements that fall into the void regions are not solved during the simulations but have an associated memory footprint. The carving of an object leads to the construction of an incomplete octree. An octree is incomplete if there are non-leaf subtrees with one or more missing children. Finally, there has been limited work in developing octree-based mesh generation to efficiently solve PDEs over complex geometries. As stated earlier, carving out affords multiple advantages (explored in this paper) at the cost of a voxelated boundary of the object. We circumvent the voxelated boundary issue via an immersed boundary (IBM) formulation on this carved-out octree. 

\added{An alternate approach has been to use two-tier meshes \cite{hhg04,BursteddeWilcoxGhattas11} that rely on having a top-level unstructured hexahedral mesh that conforms to the complex geometry and can independently refine (uniformly or adaptively) each hexahedral element of the top-level mesh. While this approach works well for simple shapes, like spheres \cite{sc08-seismic}, hex-meshing is non-trivial for more complex geometries \cite{viertel2019approach}. An alternative is then to use affine transforms within each top-level element but limits the ability to have isoparametrically refined elements. In contrast, our approach can take an arbitrary function to carve out the domain and is capable of on-the-fly refinement and coarsening that matches the arbitrary function within the refinement tolerance.  }
% \added{Additionally, unlike the approach in some of the previous literature \cite{bauer2021walberla,dubey2009extensible}, the refinement or selection criteria of our approach do not conform to  any block, wherein the elements of a block can only be discarded if all of them lies in the void region otherwise they have to be retained. This is important consideration as the past work by \citet{fernando2018massively} have shown the block strategy leads to a significantly higher number of degrees of freedom.} 
%The finite cell approach has a similar philosophy as this work, and prior work has explored using unstructured grids~\citep{varduhn2016tetrahedral} and regular structured grids~\citep{namburi2016crystallographic} to carve out the geometries.

In this work, we address some of the key algorithmic challenges that are important to consider for carrying out efficient carving-out within the octree framework, yet missing from the existing literature:
\begin{itemize}[topsep=3pt,leftmargin=*]
    \item Careful mathematical abstraction that ensures the correctness of the generated mesh for any given arbitrary shape. Additionally, within the correctly carved out region, it is critical to correctly mark the boundary elements and nodes to solve PDEs correctly. (see \secref{sec: mathAbstraction}) 
    \item Handling of hanging nodes is critical during the carving out operations. Specifically, no hanging nodes should be present at the boundaries. If so, the parent of these nodes can lie in the inactive region, which is discarded during tree pruning. This would result in an incorrect PDE solution. (see~\secref{createNodes})
    \item It is essential that the partitioning algorithm only looks at the active region of the octree. This ensures that FEM computations are evenly distributed and hence load-balanced. The data structure used in previous literature~\cite{xu2021octree} first builds a complete octree distributed among processors before canceling out the inactive regions. This leads to the generation of complete trees with a substantial fraction of the trees in inactive regions. (see \secref{sec: octreeConstruct})
    \item Efficient pruning of trees at coarser levels is essential. Earlier approaches first generate the complete octrees before pruning. This can lead to substantial overheads for non-cube geometries, such as an elongated channel. (see \secref{sec: octreeConstruct})
\end{itemize}
% To the best of the knowledge, this is the first attempt to address these key issues for an octree-based framework to be deployed efficiently for solving PDEs on non-cubical carved-out domains, \added{which do not rely on any top-level hexahedral meshes.
% }

\input{Images/IntroFig} 

% \textcolor{red}{\textbf{Ming-Chen: Please vet the above paragraph and add some more references. BG}}
%Our contributions in this paper are as follows: (a) we develop an efficient tree based adaptive mesh construction and 2:1 balancing algorithms that does not need to confirm to the isotropic domain (b) we compare the current approach with the \textit{immersed} method ; (c) we show the scaling of our framework till $8192$ processor; (d) we deploy it in conjunction with Variational Multiscale based stabilized Finite Element method to study the following non-trivial applications: i) accurately computing the drag coefficient on the sphere across a wide range of Reynolds numbers ($\mathcal{O}(1-10^6)$) encompassing the \emph{drag crisis}; ii) measuring the pressure drop in packed bed microfluidic biosensing device; iii) simulating the flow field in the classroom to understand the risk of risk of transmission of Coronavirus.
  
%The rest of the paper is organized as follows: we begin by introducing the target application in \secref{sec: Applications} that can be efficiently solved by the current approach; the key algorithmic developments for efficient mesh generation are presented in \secref{sec: Methods}; we showcase the advantages of generating incomplete octrees and present the scaling result in \secref{sec: Results}; we show the results of our target application in \secref{sec: ResultApplication} and finish by giving conclusion and future outlook in \secref{sec: Conclusion}.
% \end{itemize}


==> OldFiles/methods.tex <==
This section describes the methodology used to generate the tree-based grids (i.e., quadtrees in 2D, octrees in 3D) for arbitrary geometric domains. The key idea is to carve out regions from a $d$-dimensional cube that is \emph{inside} the immersed geometric object to generate the PDE solution domain (see \figref{fig:carvedFig}). In this paper, we refer to the aforementioned domain that is left after carving out as the \textit{subdomain}.  As noted above, the subdomain may be a sub-rectangle of a regular box, or it may have carved regions excluded from an $d$-dimensional cubic domain. The algorithms presented here are dimension agnostic, but for simplicity, we mainly focus on 3D-based grids (octree) unless specified otherwise.
%An octree is complete if and only if every non-leaf node in that octree has exactly 8 children. Based on the above definition, the desired octree for a subdomain can be \textit{incomplete}, since it can have non-leaf nodes with missing children. 

%\subsection{Notation}
%\label{subsec:notation}

%Given that large regions of the isotropic domain may be irrelevant to the problem, the goal is to have linear computational complexity keep computational complexity linear with the number of unknowns in the subdomain. Ideally, the void subtrees would be pruned away, so that they do not count towards computational work or storage costs.

Previous work~\citep{sundar2008bottom,BursteddeWilcoxGhattas11,fernando2017machine,neilsen2018massively,ishii2019solving} have demonstrated efficient methods to construct 2:1-balanced complete octrees and additional data structures to perform efficient numerical computations at a large scale. These methods order the octants of the octree using a space-filling curve (SFC) (such as the Hilbert or Morton curve) to achieve better memory accesses locality and improved distributed-memory domain decomposition. This paper presents parallel algorithms to extend numerical computations on incomplete octrees.


%%% Highlight what is different when we deal with incomplete octrees, and why traditional approaches of constructing, balancing and meshing will be much harder. 
%%% \colorbox{pink}{TODO} Also briefly describe the D4 approach to subDA and the disadvantages of that approach. 

\subsection{Specification of the Subdomain}\label{sec: mathAbstraction}

We describe an abstraction of the application-dependent arbitrary subdomains.
The subsequent tree-based algorithms depend on a user-defined function to decide whether a given point or region in space should be retained or discarded (``carved'').
In addition, the abstraction encodes enough detail for the octree algorithms to support efficient pruning during tree traversals.

Let $\Omega = C \cup C'$ be a cube comprised of two disjoint subsets:
a closed \textit{carved} set $C \subset \Omega$, and its open complement:
the \textit{retained} set $C' \equiv \Omega \setminus C$.
Enforcing $C$ as a closed set means that it contains the boundary, $\partial C \subset C$.
(Referring back to \figref{fig:carvedFig}, in 2D,
$C$ would be the disk, including $\partial C$, the red circle.)

Suppose that $\Omega$ is hierarchically partitioned according to an octree,
$\mathcal{T}$, which captures $\partial C$ well enough under some metric.
Any octant $e$ of $\mathcal{T}$ belongs to one of the following categories,
depending on the closure of the region it bounds, $\bar{e}$:
\begin{enumerate}
    \item ``carved,'' if $\bar{e} \subset C$.
    \item ``retained,'' if $\bar{e} \not \subset C$.
    \begin{enumerate}
        \item ``intercepted,'' if ``retained'' and $\bar{e} \cap C \neq \emptyset$.
        \item ``non-intercepted,'' if $\bar{e} \subset C'$
    \end{enumerate}
\end{enumerate}

The retained octants form an incomplete octree; that is,
we define $\mathcal{T}_I \equiv \mathcal{T} \setminus \{ \text{carved leafs} \}$.
The intercepted and non-intercepted sets
specify the subdomain-boundary octants
and the subdomain-internal octants, respectively.


%where the original complete octree $\mathcal{T}$ is defined. For any given set of closed geometries, $C=\{c | c\subset\Omega\}$, let $T_c$ be a octree, capturing the boundary of $c$ accurately enough for a given metric. Then we define $T_{carved} = \bigcup_{c\in C} T_c$, and the octree structure capturing $\Omega\setminus C $ (subdomain) is denoted by $T=\mathcal{T} \setminus T_{carved}$. For a given tree node $e$, let $F(e), E(e),$ and $V(e)$ denotes the faces, edges and the vertices of $e$.
%Suppose the cubic domain $\Omega$ is partitioned into two disjoint subsets, carved set $C$ and it's complement $C^\prime=\Omega \setminus C$ (retained set). $C^\prime$ is further split into two disjoint sets ``intercepted''(I) and ``non-intercepted'' (NI). The intercepted and non-intercepted sets specify the boundary and internal octants of the subdomain. 
% \begin{enumerate}
%     \item For an octant $e\in \mathcal{T}$, $\forall v \in V(e)$,  $v\in C$, then $e$ belongs to $T_{carved}$.
%     \item For an octant $e \in T$, $\forall v \in V(e)$,  $v\in C^\prime$ then $e$ is ``non-intercepted'' octant (i.e., $e\in NI$).
% \end{enumerate}



% Suppose the unit cube is partitioned into two disjoint subsets, a \textit{void} set and a \textit{nonvoid} set. A na\"{i}ve test for octants might apply a point-wise binary function (``void'' or ``nonvoid'') to the eight corners, and classify the octant as follows:
% \begin{enumerate}
%     \item All corners of a ``void'' octant are in the void set;
%     \item All corners of a ``nonvoid'' octant are in the nonvoid set;
%     \item Some corners of an ``intercepted'' octant are in each set.
% \end{enumerate}

% While the above implications are mostly true of the desired octrees, the converses may not hold.
% For example, the converse of case 1) assumes that the test is not being evaluated near the top of the tree, where large parts of the subdomain could intersect an octant without touching its corners.
% The converse of case 2) assumes that the nonvoid set is convex. As a result, simply applying a point-wise test to the corners may mis-classify some ``intercepted'' octants as ``void'' or ``nonvoid'' instead. Furthermore, special care is needed when the void/nonvoid boundary coincides with the boundary of an octant. Boundary points should be identifiable as such directly, without needing to test many nearby points.

\subsubsection{Features of the Abstraction:\;}

Defining the subdomain abstraction in this way
ensures that the octree pruning problem is well-defined.
Notice the following:

\begin{itemize}[left=0pt,topsep=0.0in]
    \item An application can specify a subdomain through a function $F(\bar{e})$,
          where $\bar{e}$ is any filled-in cube
          of zero or positive side length, such that
    \begin{align*}
    F(\bar{e}) \coloneqq \left\{
    \begin{matrix}
      \text{label(``carved'')} && \text{if~} \bar{e} \subset $C$
      \\ 
      \text{label(``retain-internal'')} && \text{if~} \bar{e} \subset $C'$
      \\
      \text{label(``retain-boundary'')} && \text{otherwise}
    \end{matrix}
    \right.
    \end{align*}
    \begin{itemize}
        \item The function $F(\bar{e})$ applies to both octants and nodal points.
        \item Points can not be classified  ``intercepted,''
              as all points are contained in the union of $C$ and $C'$.
        \item The implementation of $F$ must take care with nontrivial intersections between $\partial C$ and an element.
        Even if all vertices lie in $C$, it is possible
        for the element to be intercepted,
        and in such a case, it should be labeled as ``retain-boundary.''
        In an application, the intersection test may be as simple  or complex
        as needed by the geometry being captured.
    \end{itemize}
        
    \item $C$ is assumed closed; hence its complement, $C^\prime$, is open.
        \begin{itemize}
            \item This convention permits the robust classification
                  of a boundary element that sits flush with $\partial C$.
                  The element is labeled ``retain-boundary,''
                  while the boundary nodes are labeled ``carved.''
            
        \end{itemize}
        \item This abstraction ensures the correctness of the generated mesh, for any arbitrary geometry, along with the correct tagging of boundary elements and nodes which is of utmost important for solving PDEs correctly.
    \item It is not necessary to generate a complete octree before filtering out the       carved octants.
          If an octant is carved, all its children are carved.
          If an octant is non-intercepted, so are all its children.
          The next section describes
          how to construct incomplete octrees
          by proactively pruning subtrees during construction.
\end{itemize}


% We address all of these issues with the following conventions.
% \begin{itemize}
%     \item The void set is assumed to be closed, and its complement, the nonvoid set, is open.
%         \begin{itemize}
%             \item This convention permits robust detection of boundary points on an octant whose interior lies completely within the subdomain.
%         \end{itemize}
%     \item The application specifies the subdomain as a function $F(\bar{c})$,
%           where $\bar{c}$ is any \textit{closed} cube of zero or positive side length.
%     \begin{align*}
%     F(\bar{c}) \coloneqq \left\{
%     \begin{matrix}
%       \text{label(``void'')} && \text{if~} \bar{c} \subset Void
%       \\ 
%       \text{label(``nonvoid'')} && \text{if~} \bar{c} \subset Nonvoid
%       \\
%       \text{label(``intercepted'')} && \text{otherwise}
%     \end{matrix}
%     \right.
%     \end{align*}
    
%     \begin{itemize}
%         \item Notice that $F(\bar{c})$ applies to both octants and points.
%         \item Only octants can be classified as ``intercepted,'' as the union of void and nonvoid sets covers all points.
%         \item It is up to the application to correctly classify nontrivial intersections,
%               where the void/nonvoid boundary intercepts an octant but not its vertices.
%               The benefit is that the complexity of the intersection test may be custom-tailored
%               to the complexity of the geometry.
%     \end{itemize}
% \end{itemize}

%%% Given the filter function $F(\bar{c})$, octrees are managed according to the following policies.

% To prune a given octree whose leafs cover the subdomain, $F(\bar{c})$ is applied to each leaf:
% \begin{itemize}
%     \item The ``carved'' octants are safely discarded.
%     \item The ``retain-internal'' octants are retained and do not touch the boundary.
%     \item The ``retain-boundary'' octants are marked as boundary elements and are considered for boundary node detection.
% \end{itemize} 
% Later, once nodal points are created over the octree, boundary nodes can be identified: The ``carved'' points are marked as boundary nodes, and ``retain-interior'' points as subdomain-interior nodes.




\subsection{Octree Construction} \label{sec: octreeConstruct}

\begin{algorithm}[b!]
  \footnotesize
    \caption{ConstructUniform}
    \label{alg:construct-uniform}
    \begin{algorithmic}[1]
\Require Region $S$, SFC oracle $I$,
         final level $L$, function $F()$.
\Ensure Set $T$ of level-$L$ leafs covering subdomain, sorted by SFC.
\item[]

\If{$F(S) \neq \text{Carved}$} {\Comment Else prune}
  \If{level of $S \geq L$}
    \State $T$.push($S$)   \Comment Leaf.
    \Else
      \For{$c_\text{sfc} \leftarrow 1$ to $2^\text{dim}$}
        \Comment{Regional SFC order}
        \State $c_\text{morton} \leftarrow I$.sfc2Morton($c_\text{sfc}$)
        \State ConstructUniform($S$.child($c_\text{morton}$), $I$.child($c_\text{sfc}$))
      \EndFor
    \EndIf
\EndIf
    \end{algorithmic}
\end{algorithm}


\begin{algorithm}[t!]
 \footnotesize
    \caption{ConstructConstrained}
    \label{alg:construct-constrained}
    \begin{algorithmic}[1]
\Require Region $S$, SFC oracle $I$,
         seed octants $B$, function $F()$.
\Ensure Set $T$ of leafs, no coarser than $B$, covering the subdomain, sorted by SFC.
        
\If{$F(S) \neq \text{Carved}$} {\Comment Else prune}
  \State $L \leftarrow$ finest level in $B$
  \If{$|B| = 0$ {\bf or} level of $S \geq L$}
    \State $T$.push($S$)   \Comment Leaf.
    \Else
      \State \Comment Bucket seeds to SFC-sorted children of $S$.
      \State $l \leftarrow$ level($S$) $+1$
      \State counts[$2^\text{dim}$] $\leftarrow 0$
      \For{$b \in B$}
        \State counts[child\_num($b, l$)]$++$
      \EndFor
      \State counts[] $\leftarrow$ permute(counts, $I$)
      \State offsets[] $\leftarrow$ scan(counts)
      %%%\State
      \State \Comment Construct child subtrees in SFC order.
      \For{$c_\text{sfc} \leftarrow 1$ to $2^\text{dim}$}
        \State $c_\text{morton} \leftarrow I$.sfc2Morton($c_\text{sfc}$)
        \State $S_c \leftarrow$ $S$.child($c_\text{morton})$
        \State $I_c \leftarrow$ $I$.child($c_\text{sfc})$
        \State $B_c \leftarrow$ $B$.slice(offsets[$c_\text{sfc}$], offsets[$c_\text{sfc}+1$])
        \State ConstructConstrained($S_c$ $I_c$, $B_c$)
      \EndFor
    \EndIf
\EndIf
    \end{algorithmic}
\end{algorithm}

\begin{algorithm}[t!]
 \footnotesize
    \caption{DistributedConstructConstrained}
    \label{alg:dist-construct-constrained}
    \begin{algorithmic}[1]
\Require Distributed set of seed octants $B$, function $F()$.
\Ensure Distributed set $T$ of leafs, no coarser than $B$, covering the subdomain, sorted by SFC.

%\State DistributedTreeSort($B$)
\State \dsort($B$, load\_tol)
\Comment{\citep{ishii2019solving}}
\State $T_\text{tmp} \leftarrow$ ConstructConstrained(TreeRoot, SFC\_Root, $B$)
\State \dsort($T_\text{tmp}$, load\_tol)
\State $T_\text{local} \leftarrow$ DistributedUniqueLeafs($T_\text{tmp}$)
\State \Return $T_\text{local}$
    \end{algorithmic}
\end{algorithm}

The previous literatures have shown efficient octree algorithms to sort, construct, and traverse octrees in SFC order~\citep{sundar2008bottom,fernando2017machine,ishii2019solving}. Most of the past literature has been limited to the construction of a complete octree in an isotropic domain~\cite{sampath2008dendro,sundar2008bottom,fernando2017machine,fernando2018massively,ishii2019solving,weinzierl2019peano,macri2008octree,teunissen2018afivo,camata2013parallel}. This work builds upon them to efficiently construct the tree in presence of void regions. Algorithms~\ref{alg:construct-uniform} and~\ref{alg:construct-constrained} forms the central crux of the work, where an efficient approach for octree construction in the presence of void regions is introduced. Algorithm~\ref{alg:dist-construct-constrained} describes the partitioning algorithm based on \dsort~ to partition the trees.% among different processors.

The octree is constructed recursively in a top-down fashion
(see Algorithms~\ref{alg:construct-uniform} and~\ref{alg:construct-constrained}),
%traversing the domain analogously to \tsort \citep{fernando2017machine}.
with child subtrees being traversed in an order determined by a regional segment of the SFC.
The top of the tree represents the entire isotropic domain, while subtrees represent cubical subregions.
A given subtree is immediately pruned if it is classified as a carved region; otherwise, it is constructed.
Constructing a subtree entails either appending the subtree as a leaf
or refining it based on a refinement criterion.
In Algorithm~\ref{alg:construct-uniform}, the refinement criterion
has a depth in the tree coarser than a target depth,
whereas in Algorithm~\ref{alg:construct-constrained}, the criterion
has a depth that is coarser than a subset of seed octants.
Other criteria are possible,
e.g., intercepting the subdomain boundary
or containing more than a maximal number of points
from an initial point cloud distribution.
If a subtree is to be refined, it is split into its eight child subtrees (in 3D).
The children are permuted into the regional SFC ordering and constructed recursively.

Algorithm~\ref{alg:dist-construct-constrained} uses the octree partitioning method based on 
\dsort~\citep{fernando2017machine,ishii2019solving}
to distribute octrees in parallel. \added{\dsort{} uses \tsort~ based comparison-free search algorithm for octree construction. Instead of performing comparison-based binary searches, \tsort~ performs MSD radix sort, except that the ordering of buckets are permuted at each level according to the specified SFC. By performing a fixed number of passes over the input data in a highly localized manner, \tsort~ avoids cache misses and random memory access  leading to  better memory performance. \cite{fernando2017machine,fernando2018massively} } Since the constructed octrees from previous algorithms entail only the active regions of the isotropic domain, \dsort~ distributes only these aforementioned active portion. This is the main difference from the past approaches, where the sorting algorithm looks at the complete tree. This step is pivotal to ensure load-balanced computation. Similar to Algorithm~\ref{alg:construct-constrained},
a set of seed octants is used to control the output tree depth.
In the distributed setting, the seed octants also inform the domain decomposition so that each rank will own approximately the same number of elements.
Note that \dsort~ accepts a tunable load-balance tolerance.
A large tolerance will partition the tree at coarse levels.
A small tolerance will balance the load more evenly
at the expense of splitting coarse subtrees over multiple processes.
Once the depth-constraining seed octants have been partitioned,
each rank constructs a tree satisfying the local constraints.
Then, overlaps between trees must be resolved.
Duplicate octants are deleted.
Finer octants are preferred to coarser overlapping octants
in order to satisfy the depth constraints globally. 

\subsection{2:1 Balancing}

\begin{algorithm}[t!]
 \footnotesize
    \caption{DistributedConstruct2to1Balanced}
    \label{alg:dist-construct-balanced}
    \begin{algorithmic}[1]
\Require Distributed set of seed octants $B$, function $F()$.
\Ensure Distributed set $T$ of leafs, no coarser than $B$, covering the subdomain, obeying 2:1-balance constraint, sorted by SFC.

\State $T_1 \leftarrow$ DistributedConstructConstrained($B$, $F$)
\State $T_2 \leftarrow$ BottomUpConstrainNeighbors($T_1$)  \Comment{$F$ not applied}
\State $T_3 \leftarrow$ DistributedConstructConstrained($T_2$, $F$)
\State \Return $T_3$
    \end{algorithmic}
\end{algorithm}

\begin{algorithm}[t!]
 \footnotesize
    \caption{BottomUpConstrainNeighbors}
    \label{alg:constrain-neighbors}
    \begin{algorithmic}[1]
\Require Unbalanced leafs $T_1$.
\Ensure Balanced seeds $T_2$.

\State $T_\text{aux}$[] $\leftarrow$ stratify $T_1$ by levels, from finest to coarsest
\For {level $l$ from finest to coarsest}
    \For {$t \in T_\text{aux}$[$l$]}
      \For {$n \in$ MakeNeighbors(MakeParent($t$))}
        \State $T_\text{aux}$[$l-1$].add\_unique($n$)
      \EndFor
    \EndFor
\EndFor
\State $T_2 \leftarrow$ concatenate($T_\text{aux}$)
\State \Return $T_2$
    \end{algorithmic}
\end{algorithm}

\input{Plots/balanceFig}
In a \textit{2:1-balanced} octree (\figref{fig:aux_bal}), a pair of octants sharing any parts of their boundaries
may differ in scale by at most a factor of 2:1. In other words, they may differ by at most one level in the tree.
Numerical computations on the octree grid are simpler in terms of the neighborhood data structures if the octree obeys the 2:1-balancing constraint .

We take a bottom-up approach to transform a given linear octree into a 2:1-balanced octree, based on the local block balancing method similar to the one by~\citet{sundar2008bottom}.
In our method (Algorithms~\ref{alg:dist-construct-balanced} and~\ref{alg:constrain-neighbors}),
the input octree comprises an initial set of seed octants.
The seed set is iteratively updated from the finest to the coarsest level.
For each seed octant, the neighbors of its parent octant are added to the next-coarser level of seeds.
Duplicate octants are removed from the next level before proceeding.
Finally, after all the levels have been processed, a new linear octree is constructed such that each seed octant
becomes either a leaf or an ancestor subtree in the output octree.
Thus the final seed set controls the resolution of the new octree,
ensuring the result is 2:1-balanced. It is important not to preemptively discard the carved octants,
which are generated as neighbors of parents of seed octants.
Otherwise, two leaf octants of 4:1 or greater ratio could meet in a carved region.
% Nonetheless, the overhead from ``void'' octants will be kept to a minimum if they are discarded
% during, or immediately following, each tree construction step.

%\subsection{Creation of Nodal Points (Continuous Galerkin)}
\subsection{Embedding Nodal Information}
\label{createNodes}
Each leaf octant in a linear 2:1-balanced octree represents an element in the FEM adaptive grid.
For a given $p$-refinement, there are $(p+1)^3$ nodes per element (in 3D).
Nodal points on the boundary of an element will be shared with same-level neighboring elements.
Nodes incident on a coarser-level neighbor is considered \textit{hanging nodes} (\figref{fig:aux_bal}).
The value of a hanging node is dependent on the values of the nodes on the coarser face or edge.
Therefore, the set of independent degrees of freedom (DOFs) on the FEM grid (underpinning a grid vector)
is defined by enumerating the unique, non-hanging nodes.

First, we loop over all elements and generate the node coordinates
with a spacing of $\left( \text{length}_\text{element} \right) / p$ in each axis.
(Nodes labeled as ``carved'' are marked as subdomain boundary nodes.)
%Inter-element nodal coordinates in the grid will have been duplicated.
The set of unique nodes is found by executing \tsort{~} on the nodal coordinates and removing duplicates.

An extra step is required to detect and discard hanging nodes.
In an isotropic domain, a hanging node
has fewer instances than the number expected
%are detected by counting the number of instances,
%which is less than the number expected
for an ordinary node as a function of the coordinate and grid level.
With user-specified geometry, however, the expected number of instances is nontrivial to compute.
Our solution is to explicitly ``cancel'' possible hanging nodes using temporary \textit{cancellation nodes}.
The cancellation nodes are generated on the edges and faces of elements in between the ordinary nodes,
anticipating the coordinates of hanging nodes from hypothetical finer neighbors.
After sorting, every coordinate is occupied by a mix of ordinary and cancellation nodes.
If a cancellation node is present, then the coordinate is incident on a coarser edge or face, and thus the node is hanging; the node is discarded.
Otherwise, no cancellation node is present, and the coordinate is enumerated as an ordinary node.
Thus we enumerate exactly the nodes which define a grid vector. Note that ensuring the absence of hanging nodes at the carved boundary is essential for accurate PDE solutions.


%%\mi{remove claims on mem efficiency}
\subsection{Matrix-free, Traversal-based~\mvec}
We implement a traversal-based matrix-vector multiplication to perform matrix-free computations, which extends the methods by~\citet{ishii2019solving} to incomplete trees.

\paragraph{Matrix free:\;}
The global matrix is defined as a summation of local elemental matrices,
where the summation is due to common nodal points being shared by neighboring elements.
We are able to apply the global operator to a grid vector without explicitly assembling the global matrix.
Instead, we perform a series of elemental matrix-vector multiplications,
and use the octree structure to compose the results.

\paragraph{Traversal-based:\;}(\figref{fig:traversal})
The elemental matrix couples elemental nodes in a global input grid vector with equivalent elemental nodes in a global output grid vector.
Within a grid vector, the nodes pertaining to a particular element are generally not stored contiguously.
If one were to read and write to the elemental nodes using an element-to-node map, the memory accesses would require indirection:
$v_{glob}[map[e*npe + i]] += v_{loc}$.
Not only do element-to-node maps cause indirect memory accesses;
the maps become complicated to build if the octree is incomplete due to complex geometry.
We take an alternative approach that obviates the need for element-to-node maps.
Instead, through top-down and bottom-up traversals of the octree,
we ensure that elemental nodes are stored contiguously in a leaf,
and there apply the elemental matrix. 

%%%\textbf{top-down}
The idea of the top-down phase is to selectively copy nodes
from coarser to finer levels until the leaf level,
wherein the selected nodes are exactly the elemental nodes.
Starting at the root of the tree, we have all the nodes in the grid vector.
We create buckets for all child subtrees.
Looping through the nodes, a node is copied into a bucket if the node is incident on the child subtree corresponding to that bucket.
A node that is incident on multiple child subtrees will be duplicated.
By recursing on each child subtree and its corresponding bucket of incident nodes, we eventually reach the leaf level.

%%%\textbf{leaf}
Once the traversal reaches a leaf octant, the elemental nodes have been copied into a contiguous array.
The elemental matrix-vector product is computed directly, without the use of an element-to-node map.
The result is stored in a contiguous output buffer the same size as the local elemental input vector.

%%%\textbf{bottom-up}
After all child subtrees have been traversed, the bottom-up phase returns results from a finer to a coarser level.
The parent subtree nodes are once again bucketed to child subtrees,
but instead of the parent values being copied, the values of nodes from each child are accumulated into a parent output array.
That is, for any node that is incident on multiple child subtrees, the values from all node instances are summed to a single value.
The global matrix-vector product is completed after the bottom-up phase executes at the root of the octree.

Distributed memory is supported by two slight augmentations.
Firstly, the top-down and bottom-up traversals operate on ghosted vectors.
Therefore ghost exchanges are required before and after each local traversal.
Secondly, the traversals are restricted to subtrees containing the owned octants.
The list of owned octants is bucketed top-down, in conjunction with the bucketing of nodal points.
A child subtree is traversed recursively only if one or more owned octants are bucketed to it. Note that because the traversal path is restricted by a list of existing octants,
the traversal-based~\mvec~ gracefully handles incomplete octrees without special treatment.

\input{Plots/traversal}
% \paragraph{Extension to incomplete trees}
% All the child subtrees in a complete octree overlap automatically with the domain,
% and therefore all child subtrees would be traversed recursively.
% In \citep{ishii2019solving}, this assumption allowed the authors to
% discard the list of octants underpinning the FEM grid,
% and still perform traversal-based {\mvec}s on the set of nodal points.
% For incomplete trees, however, the explicit octant list must be retained.
% The octant list is bucketed top-down, in conjunction with the bucketing of nodal points.
% A child subtree is traversed recursively only if one or more subdomain octants are bucketed to it.


\begin{remark}
The traversal based~\mvec~ is designed to expose memory locality suited for deep memory hierarchies inherent in modern day clusters and accelerators like GPUs. In this work, we focus on distributed memory parallelism; the implementation on accelerators is deferred to future work.
\end{remark}

\subsection{Traversal-based Matrix Assembly}

In the previous section, we described~\mvec~ procedure that employs a tree traversal, requiring neither element-to-node maps nor global matrix assembly. In this section, we describe the matrix assembly procedure for computing the global sparse matrix. The efficient computation of matrix assembly becomes particularly important for the problems whose convergence heavily depends on the preconditioners.

% addition, we also support a traversal-based matrix assembly for the global sparse matrix. 

To implement assembly, we have leveraged PETSc interface~\citep{petsc-web-page,petsc-efficient},
which only requires a sequence of entries
$(\text{id}_\text{row}, \text{id}_\text{col}, \text{val})$,
and can be configured to add entries with duplicate indices~\citep{petsc-user-ref}. Note that any other distributed sparse-matrix library can be supported in a similar fashion.

The remaining task is to associate the correct global node indices
with the rows and columns of every elemental matrix.
We use an octree traversal to accomplish this task.
Similar to the traversal-based~\mvec,
nodes are selectively copied from coarser to finer levels, recursively,
until reaching the leaf, wherein the elemental nodes are contiguous.
Note that integer node ids are copied instead of floating-point values from a grid vector.
At the leaf, an entry of the matrix is emitted
for every row and column of the elemental matrix,
using the global row and column indices instead of the elemental ones.
No bottom-up phase is required for assembly,
as PETSc handles the merging of multi-instanced entries.

% \subsection{Distributed Memory parallelism}

% %%% Describe how shared memory and distributed memory parallelism are realized.

% \subsection{Additional considerations}

% %%% Any other issues that we had to add support for, like boundary conditions etc.

==> OldFiles/roofline.tex <==
\input{Plots/roofline}
\added{~\figref{fig:roofline} shows the single core roofline plot for the elemental ~\mvec~ computation of Poisson operator using linear and quadratic basis function on ~\Frontera. Overall, we can see that the code is memory bound as is common for finite element codes. We observe higher arithmetic intensity \footnote{AI is measured as the amount of floating point operations performed per byte of data loaded into the memory.}
(AI) for quadratic (0.121) as compared to linear (0.072) elements. The amount of data needed for ~\mvec~ computation grows as $\mathcal{O}((p+1)^d)$ whereas the ~\mvec~ computation complexity grows as $\mathcal{O}(d(p+1)^{d+1})$. Therefore, AI tends to increase with polynomial order, which explains the observed behavior. We are able to achieve a performance of about 4 GFLOP/s using linear basis function and 7 GFLOP/s using quadratic basis functions for two different meshes, which corresponds to a bandwidth of approximately 60 GB/s as shown by the green lines. We note that we have not used any hand-coded explicit vectorization to ensure the portability of the code across various platforms and relied on compiler-directed vectorization. We would like to explore some future avenues from the code optimization point of view pertaining to more efficient cache blocking techniques and architecture-specific efficient vectorized implementation of tensor products.
}


==> OldFiles/scaling.tex <==

\added{We evaluated the strong and weak scaling performance of our traversal-based \mvec~ using linear and quadratic elements on the \Frontera~ supercomputer for two different cases: a) an elongated channel of dimension $16 \times 1 \times 1$, b) a spherical region carved out from the cube. We individually timed the execution of major components of \mvec, namely top-down and bottom-up traversal, leaf \mvec~ to compute the elemental operators, malloc and communication cost. It must be noted that for any PDE solver, \mvec~ is the basic building block and determines the overall parallel performance and scalability. 
}
\added{We highlight some important points regarding the experimental setup for performing the scaling studies and the interpretability of the scaling results:
\begin{itemize}[left=0in]
    \item \textit{Strong Scaling:\;} For each of the strong scaling cases, we generated a fixed mesh defined by different refinement levels in different regions of interest. When comparing the mesh with linear and quadratic elements, the total number and distribution of elements in a given mesh is the same not only at a global level but also locally at each processor level. Note that the partitioning algorithm \dsort~ is agnostic to the underlying element order and distributes the element at the octant level  before the nodal information is encoded~\footnote{More formally, consider a mesh $M$ with $N$ global elements distributed over $p$ processor. If we globally number the elements of mesh from $0 \cdots N-1$, then if a processor $k, k\leq p$, receives $m_i \cdots m_k$ ($m_i$'s being the global element number)  elements for linear, $0 \leq m_i \leq m_k \leq N-1$, then the processor $k$ for quadratic mesh will also receive the same sequence of elements $m_i \cdots m_k$.}.
    \item However, the total number of DOF and problem size grows as $\mathcal{O}((p+1)^d)$ for an arbitrary order $p$ and dimension $d$~\footnote{Every element has $\mathcal{O}((p+1)^d)$ nodes (Refer \secref{createNodes}).}. Hence, the mesh with linear and quadratic elements have different computation and communication complexity. For instance, both linear and quadratic mesh for channel strong scaling study have 13.5M elements. But  the linear element mesh has 13.7M DOFs, whereas the quadratic has 109.1M DOFs.
    \item \textit{Weak Scaling:\;} For the weak scaling runs, with an increase in the number of processors, we increase the refinement level in the regions of interest in such a way that the average number of elements per processor remains the same. Similar to the strong scaling, for a given number of processors, the total number and distribution of elements are the same for both linear and quadratic basis functions both globally and locally. Hence, the quadratic mesh has a greater number of DOF compared to the linear one.
    \item In all the scaling figures (\figref{fig:strong-scaling} --\figref{fig:weak-scalingSphere}), for a given number of processors, the left bar corresponds to the \mvec~ execution profile for the linear elements, and the right bar corresponds to the execution profile of the quadratic elements. The total execution time for the linear elements is shown by solid blue lines and red dashed lines for the quadratic.
\end{itemize}
}
\subsubsection{Scaling results for the channel:\;}\label{sec:channelScaling}
The incomplete octrees representing $16 \times 1 \times 1$ elongated channel, with greater refinement on the boundary and minimal refinement on the interior, are generated to carry out the scaling studies. This is representative of the common cases that arise in the boundary-dominated physical phenomena. Each scaling run was repeated for linear and quadratic hexahedral grids.

\added{For the strong scaling runs, we generated octree mesh with 13M elements for linear and quadratic basis functions. Both linear and quadratic mesh is similar at the elemental level. \figref{fig:strong-scaling}  shows the strong scaling behavior in terms of parallel cost (Run time $\times$ number of cores) for both the linear and quadratic basis functions. A constant line would mean ideal strong scaling efficiency. For the linear mesh, \mvec~ execution time decreased from 2.87 s on 224 processors to 0.027 s on 28K processors, resulting in 81\% parallel efficiency for 128 fold increase in processor count. Similarly, for the quadratic mesh, we see a reduction in \mvec~ execution time from 13.5 s on 224 processors to 0.1 s on 28K processors, resulting in 90\% parallel efficiency. The overall theoretical complexity for \mvec~ for a given element of order $p$ has been shown to scale as $\mathcal{O}( d(p+1)^{d+1})$. We see a factor of 4.2 $\times$ increase in \mvec~ execution time for quadratic element $(p=2)$ over linear $(p=1)$, which is within the theoretical bounds.}

\added{
For the weak scaling runs, we created grids with a fixed grain size of about 35K elements per core and timed \mvec~ execution time. The coarsest mesh consists of 981K elements on 28 processors  with 1.02M DOFs for linear and 8.01M DOFs for quadratic element, whereas the finest mesh consists of 502M elements on a 14K processors with 505M DOFs for linear and 4 billion DOFs for quadratic elements.  \figref{fig:weak-scaling} plots the mean execution of the  \mvec~ averaged over 100 iterations as a function of the number of cores. A constant execution time would imply ideal weak scaling efficiency. We observed a slowly growing weak-scaled execution time. Overall the time increased from about 1.58 s on 28 cores to 1.9 s on 14 K cores for linear elements (82\% weak scaling efficiency) and 7.04 s to 8.04 s for quadratic elements (86\% weak scaling efficiency).}


% \input{Plots/channelScaling}
%%%
%%% Strong scaling
%%%
\begin{figure}[tbh]
  \centering
  \begin{tikzpicture}
  \begin{axis}[
  ybar stacked, bar width=5pt,    
  xlabel={Number of cores $\rightarrow$},
  ylabel={\small{Parallel cost  (cores $\cdot$ s) $\rightarrow$}},
%   ylabel=A very long\\long\\text as a label,
   symbolic x coords={224,448,896,1792,3584,7168,14336,28672},width=8.8cm,height=4cm,
  xtick = data, 
  ymin=0,
  ymax = 1.99,
  x tick label style={font=\small},
  legend pos=north west,grid=major,legend style={at={(0.5,1.0)},
		anchor=south,legend columns=5}]

  % linear
  \addplot [fill=div_d1] [bar shift=-.125cm] table[x={npes} , y expr={\thisrow{topdown(mean)}*\thisrow{npes}/2240} ]{Data/Channel/LinearSS.txt};
  \addplot [fill=div_d2] [bar shift=-.125cm]  table[x={npes}, y expr={\thisrow{bottomup(mean)}*\thisrow{npes}/2240} ]{Data/Channel/LinearSS.txt};
  \addplot [fill=div_d3] [bar shift=-.125cm]  table[x={npes}, y expr={\thisrow{elemental(mean)}*\thisrow{npes}/2240} ]{Data/Channel/LinearSS.txt};
  \addplot [fill=div_d4] [bar shift=-.125cm]  table[x={npes}, y expr={(\thisrow{matvec(mean)}-\thisrow{elemental(mean)}-\thisrow{bottomup(mean)}-\thisrow{topdown(mean)})*\thisrow{npes}/2240} ]{Data/Channel/LinearSS.txt};
  \addplot [fill=div_d5] [bar shift=-.125cm] table[x={npes}, y expr={\thisrow{ghostexchange(mean)}*\thisrow{npes}/2240} ]{Data/Channel/LinearSS.txt};
  
  \makeatletter
  \newcommand\resetstackedplotsA{
  \makeatletter
  \pgfplots@stacked@isfirstplottrue
  \makeatother
  \addplot [forget plot,draw=none] coordinates{(224,0) (448,0) (896,0) (1792,0) (3584,0) (7168,0) (14336,0) (28672,0)};
  }
  \makeatother
  \resetstackedplotsA
  % quadratic
 \addplot [fill=div_d1] [bar shift=.125cm] table[x={npes} , y expr={\thisrow{topdown(mean)}*\thisrow{npes}/2240} ]{Data/Channel/QuadraticSS.txt};
  \addplot [fill=div_d2] [bar shift=.125cm]  table[x={npes}, y expr={\thisrow{bottomup(mean)}*\thisrow{npes}/2240} ]{Data/Channel/QuadraticSS.txt};
  \addplot [fill=div_d3] [bar shift=.125cm]  table[x={npes}, y expr={\thisrow{elemental(mean)}*\thisrow{npes}/2240} ]{Data/Channel/QuadraticSS.txt};
  \addplot [fill=div_d4] [bar shift=.125cm]  table[x={npes}, y expr={(\thisrow{matvec(mean)}-\thisrow{elemental(mean)}-\thisrow{bottomup(mean)}-\thisrow{topdown(mean)})*\thisrow{npes}/2240} ]{Data/Channel/QuadraticSS.txt};
  \addplot [fill=div_d5] [bar shift=.125cm] table[x={npes}, y expr={\thisrow{ghostexchange(mean)}*\thisrow{npes}/2240} ]{Data/Channel/QuadraticSS.txt};
  
  \legend{\small{top-down},\small{bottom-up}, \small{leaf \mvec}, \small{malloc}, \small{communicate}}
  \end{axis}
     \begin{axis}[ axis y line=none,axis x line = none,symbolic x coords={224,448,896,1792,3584,7168,14336,28672},width=8.8cm,height=4cm,
        xtick = data,ymin=0,ymax=1.99,legend style={at={(0.3,0.8)},
		anchor=south,legend columns=2}] %second axis, function 
      %\addplot[sq_b1,thick]  table[x={npes}, y expr={(\thisrow{matvec(max)} + \thisrow{ghostexchange(max)}) /(\thisrow{matvecNumNodes}/\thisrow{npes})} ]{dat/dkt_matvec_adap_ws_e1_stampede2.dat};
      %\addplot[sq_r1,thick,dashed]  table[x={npes}, y expr={(\thisrow{matvec(max)} + \thisrow{ghostexchange(max)}) /(\thisrow{matvecNumNodes}/\thisrow{npes})} ]{dat/dkt_matvec_adap_ws_e2_stampede2.dat};
      
      \addplot[sq_b1,ultra thick]  table[x={npes}, y expr={(\thisrow{matvec(mean)} + \thisrow{ghostexchange(mean)})*\thisrow{npes}/2240} ]{Data/Channel/LinearSS.txt};
      \addplot[sq_r1,ultra thick,dashed]  table[x={npes}, y expr={(\thisrow{matvec(mean)} + \thisrow{ghostexchange(mean)})*\thisrow{npes}/2240} ]{Data/Channel/QuadraticSS.txt};
      
      \legend{\small{linear},\small{quadratic}}
  
%%%    \begin{axis}[ axis y line=none,axis x line = none,symbolic x coords={16,32,64,128,256,512,1024,2048,4096,8192},width=9cm,height=5cm,
%%%         xtick = data,legend pos={north east}] %second axis, function 
%%%       \addplot[sq_b1,thick]  table[x={npes}, y expr={(\thisrow{matvec_eff} + \thisrow{ghostexchange_eff}) /(100.0)} ]{Data/strong_effc_p1.tsv};
%%%       \addplot[sq_r1,thick,dashed]  table[x={npes}, y expr={(\thisrow{matvec_eff} + \thisrow{ghostexchange_eff}) /(100.0)} ]{Data/strong_effc_p2.tsv};
%%%       \legend{linear,quadratic}
%%%   \end{axis}  
  \end{axis}
  \end{tikzpicture}
  \caption{\added{\textit{Strong scaling for channel case.\;} Parallel cost evaluated with the 3D Poisson \mvec~ on \Frontera~ supercomputer. Problem size was fixed at 13M elements (13.7M unknowns for linear and 109.1M unknowns for quadratic)}}
  \label{fig:strong-scaling}
\end{figure}


%%%
%%% Weak scaling
%%%
\begin{figure}[tbh]
  \centering
  \begin{tikzpicture}
  \begin{axis}[
  ybar stacked, bar width=5pt,    
  xlabel={Number of cores $\rightarrow$},
  ylabel={Time (s) $\rightarrow$ },
  ymin=0.0,
  ymax=9.9,
  symbolic x coords={28,224,1792,14336},width=8.8cm,height=4cm,
  xtick = data, 
%   x tick label style={rotate=0, anchor=east, align=right},
%   x tick label style={rotate=0},
  legend pos=north west,grid=major,legend style={at={(0.5,1.0)},
		anchor=south,legend columns=5}]

  % linear
  \addplot [fill=div_d1] [bar shift=-.101cm] table[x={npes} , y expr={\thisrow{topdown(mean)}} ]{Data/Channel/LinearWS.txt};
  \addplot [fill=div_d2] [bar shift=-.101cm]  table[x={npes}, y expr={\thisrow{bottomup(mean)}} ]{Data/Channel/LinearWS.txt};
  \addplot [fill=div_d3] [bar shift=-.101cm]  table[x={npes}, y expr={\thisrow{elemental(mean)}} ]{Data/Channel/LinearWS.txt};
  \addplot [fill=div_d4] [bar shift=-.101cm]  table[x={npes}, y expr={(\thisrow{matvec(mean)}-\thisrow{elemental(mean)}-\thisrow{bottomup(mean)}-\thisrow{topdown(mean)})} ]{Data/Channel/LinearWS.txt};
  \addplot [fill=div_d5] [bar shift=-.101cm] table[x={npes}, y expr={\thisrow{ghostexchange(mean)}} ]{Data/Channel/LinearWS.txt};
  
  \makeatletter
  \newcommand\resetstackedplotsThree{
  \makeatletter
  \pgfplots@stacked@isfirstplottrue
  \makeatother
   \addplot [forget plot,draw=none] coordinates{(28,0) (224,0) (1792,0) (14336,0)};
 }
  \makeatother
  \resetstackedplotsThree
  % quadratic
  \addplot [fill=div_d1] [bar shift=+.101cm] table[x={npes} , y expr={\thisrow{topdown(mean)}} ]{Data/Channel/QuadWS.txt};
  \addplot [fill=div_d2] [bar shift=+.101cm]  table[x={npes}, y expr={\thisrow{bottomup(mean)}} ]{Data/Channel/QuadWS.txt};
  \addplot [fill=div_d3] [bar shift=+.101cm]  table[x={npes}, y expr={\thisrow{elemental(mean)}} ]{Data/Channel/QuadWS.txt};
  \addplot [fill=div_d4] [bar shift=+.101cm]  table[x={npes}, y expr={(\thisrow{matvec(mean)}-\thisrow{elemental(mean)}-\thisrow{bottomup(mean)}-\thisrow{topdown(mean)})} ]{Data/Channel/QuadWS.txt};
  \addplot [fill=div_d5] [bar shift=+.101cm] table[x={npes}, y expr={\thisrow{ghostexchange(mean)}} ]{Data/Channel/QuadWS.txt};
  \legend{\small{top-down}, \small {bottom-up}, \small {leaf \mvec},\small {malloc}, \small {communicate}}
  \end{axis}
  
    \begin{axis}[ axis y line=none,axis x line = none,symbolic x coords={28,224,1792,14336},width=8.8cm,height=4cm,
        xtick = data,ymin=0,ymax=10.0,legend style={at={(0.3,0.8)},
		anchor=south,legend columns=2}] %second axis, function 
%       %\addplot[sq_b1,thick]  table[x={npes}, y expr={(\thisrow{matvec(max)} + \thisrow{ghostexchange(max)}) /(\thisrow{matvecNumNodes}/\thisrow{npes})} ]{dat/dkt_matvec_adap_ws_e1_stampede2.dat};
%       %\addplot[sq_r1,thick,dashed]  table[x={npes}, y expr={(\thisrow{matvec(max)} + \thisrow{ghostexchange(max)}) /(\thisrow{matvecNumNodes}/\thisrow{npes})} ]{dat/dkt_matvec_adap_ws_e2_stampede2.dat};
      
      \addplot[sq_b1,ultra thick]  table[x={npes}, y expr={(\thisrow{matvec(mean)} + \thisrow{ghostexchange(mean)})} ]{Data/Channel/LinearWS.txt};
      \addplot[sq_r1,ultra thick,dashed]  table[x={npes}, y expr={(\thisrow{matvec(mean)} + \thisrow{ghostexchange(mean)})} ]{Data/Channel/QuadWS.txt};
      \legend{\small{linear},\small{quadratic}}
  \end{axis}  
  \end{tikzpicture}
  
  \caption{\textit{Weak scaling run time for channel case:\;} Execution time of 3D Poisson \mvec~ on \Frontera~ supercomputer, for a fixed grain size of about 35K elements per core. }
  \label{fig:weak-scaling}
\end{figure}


%%% \begin{figure}[tbh]
%%%   \centering
%%%   \begin{tikzpicture}
%%%   \begin{axis}[
%%%   ybar stacked, bar width=5pt,    
%%%   xlabel={number of cores $\rightarrow$},
%%%   ylabel={time(s) $\rightarrow$ },
%%%   ymax=9e-2,
%%%   symbolic x coords={1,2,4,8,16,32,64,128,256},width=9cm,height=5cm,
%%%   xtick = data, 
%%%   x tick label style={rotate=45, anchor=east, align=right},legend pos=north west,grid=major,legend style={at={(0.55,0.7)},
%%% 		anchor=south,legend columns=3}]
%%% 
%%%   % linear
%%%   \addplot [fill=div_d1] [bar shift=-.125cm] table[x={npes} , y expr={\thisrow{topdown(mean)}/10.0} ]{Data/weak_p1_2K.txt};
%%%   \addplot [fill=div_d2] [bar shift=-.125cm]  table[x={npes}, y expr={\thisrow{bottomup(mean)}/10.0} ]{Data/weak_p1_2K.txt};
%%%   \addplot [fill=div_d3] [bar shift=-.125cm]  table[x={npes}, y expr={\thisrow{elemental(mean)}/10.0} ]{Data/weak_p1_2K.txt};
%%%   \addplot [fill=div_d4] [bar shift=-.125cm]  table[x={npes}, y expr={(\thisrow{matvec(mean)}-\thisrow{elemental(mean)}-\thisrow{bottomup(mean)}-\thisrow{topdown(mean)})/10.0} ]{Data/weak_p1_2K.txt};
%%%   \addplot [fill=div_d5] [bar shift=-.125cm] table[x={npes}, y expr={\thisrow{ghostexchange(mean)}/10.0} ]{Data/weak_p1_2K.txt};
  
%%%   \makeatletter
%%%   \newcommand\resetstackedplotsThree{
%%%   \makeatletter
%%%   \pgfplots@stacked@isfirstplottrue
%%%   \makeatother
 %%%  \addplot [forget plot,draw=none] coordinates{(1,0) (2,0) (4,0) (8,0) (16,0) (32,0) (64,0) (128,0) (256,0)};
%%%   }
%%%   \makeatother
%%%   \resetstackedplotsThree
%%%   % quadratic
%%%   \addplot [fill=div_d1] [bar shift=+.125cm] table[x={npes} , y expr={\thisrow{topdown(mean)}/10.0} ]{Data/weak_p2_2K.txt};
%%%   \addplot [fill=div_d2] [bar shift=+.125cm]  table[x={npes}, y expr={\thisrow{bottomup(mean)}/10.0} ]{Data/weak_p2_2K.txt};
%%%   \addplot [fill=div_d3] [bar shift=+.125cm]  table[x={npes}, y expr={\thisrow{elemental(mean)}/10.0} ]{Data/weak_p2_2K.txt};
%%%   \addplot [fill=div_d4] [bar shift=+.125cm]  table[x={npes}, y expr={(\thisrow{matvec(mean)}-\thisrow{elemental(mean)}-\thisrow{bottomup(mean)}-\thisrow{topdown(mean)})/10.0} ]{Data/weak_p2_2K.txt};
%%%   \addplot [fill=div_d5] [bar shift=+.125cm] table[x={npes}, y expr={\thisrow{ghostexchange(mean)}/10.0} ]{Data/weak_p2_2K.txt};
  
%%%   \legend{\small top-down, bottom-up, leaf \mvec, malloc, communicate}
%%%   \end{axis}
  
%%% %   \begin{axis}[ axis y line=none,axis x line = none,symbolic x coords={1,2,4,8,16,32,64,128,256,512,1024,2048},width=9cm,height=5cm,
%         xtick = data,legend pos={north east}] %second axis, function 
%       \addplot[sq_b1,thick]  table[x={npes}, y expr={(\thisrow{matvec(mean)} + \thisrow{ghostexchange(mean)}) /(10.0)} ]{Data/weak_p1_2K.txt};
%       \addplot[sq_r1,thick,dashed]  table[x={npes}, y expr={(\thisrow{matvec(mean)} + \thisrow{ghostexchange(mean)}) /(10.0)} ]{Data/weak_p2_2K.txt};
%       %\legend{linear,quadratic}
%   \end{axis}  
  
%%%   \end{tikzpicture}
  
%%%   \caption{\textit{Weak scaling.} Weak scaling result on \Frontera~ supercomputer for a grain size of around 1K per processor. }
%%%   \label{fig:weak-scaling}
%%% \end{figure}






% \begin{figure}[tbh]
%   \centering
%   \begin{tikzpicture}
%   \begin{axis}[
%   ybar stacked, bar width=5pt,    
%   xlabel={number of cores $\rightarrow$},
%   ylabel={time(s) $\rightarrow$ },symbolic x coords={512,1024,2048,4096,8192},width=9cm,height=5cm,
%   xtick = data, 
%   x tick label style={rotate=45, anchor=east, align=right},legend pos=north west,grid=major,legend style={at={(0.55,1.0)},
% 		anchor=south,legend columns=3}]

%   % linear
%   \addplot [fill=div_d1] [bar shift=-.125cm] table[x={npes} , y expr={\thisrow{topdown(mean)}/10.0} ]{Data/strong_8K_p1.tsv};
%   \addplot [fill=div_d2] [bar shift=-.125cm]  table[x={npes}, y expr={\thisrow{bottomup(mean)}/10.0} ]{Data/strong_8K_p1.tsv};
%   \addplot [fill=div_d3] [bar shift=-.125cm]  table[x={npes}, y expr={\thisrow{elemental(mean)}/10.0} ]{Data/strong_8K_p1.tsv};
%   \addplot [fill=div_d4] [bar shift=-.125cm]  table[x={npes}, y expr={(\thisrow{matvec(mean)}-\thisrow{elemental(mean)}-\thisrow{bottomup(mean)}-\thisrow{topdown(mean)})/10.0} ]{Data/strong_8K_p1.tsv};
%   \addplot [fill=div_d5] [bar shift=-.125cm] table[x={npes}, y expr={\thisrow{ghostexchange(mean)}/10.0} ]{Data/strong_8K_p1.tsv};
  
%   \makeatletter
%   \newcommand\resetstackedplotsThree{
%   \makeatletter
%   \pgfplots@stacked@isfirstplottrue
%   \makeatother
%   \addplot [forget plot,draw=none] coordinates{ (512,0) (1024,0) (2048,0) (4096,0) (8192,0)};
%   }
%   \makeatother
%   \resetstackedplotsThree
%   % quadratic
%   \addplot [fill=div_d1] [bar shift=+.125cm] table[x={npes} , y expr={\thisrow{topdown(mean)}/10.0} ]{Data/strong_8K_p2.tsv};
%   \addplot [fill=div_d2] [bar shift=+.125cm]  table[x={npes}, y expr={\thisrow{bottomup(mean)}/10.0} ]{Data/strong_8K_p2.tsv};
%   \addplot [fill=div_d3] [bar shift=+.125cm]  table[x={npes}, y expr={\thisrow{elemental(mean)}/10.0} ]{Data/strong_8K_p2.tsv};
%   \addplot [fill=div_d4] [bar shift=+.125cm]  table[x={npes}, y expr={(\thisrow{matvec(mean)}-\thisrow{elemental(mean)}-\thisrow{bottomup(mean)}-\thisrow{topdown(mean)})/10.0} ]{Data/strong_8K_p2.tsv};
%   \addplot [fill=div_d5] [bar shift=+.125cm] table[x={npes}, y expr={\thisrow{ghostexchange(mean)}/10.0} ]{Data/strong_8K_p2.tsv};
  
%   \legend{\small top-down, bottom-up, leaf \mvec, malloc, communicate}
%   \end{axis}
  
%   \begin{axis}[ axis y line=none,axis x line = none,symbolic x coords={512,1024,2048,4096,8192},width=9cm,height=5cm,
%         xtick = data,legend pos={north east}] %second axis, function 
%       \addplot[sq_b1,thick]  table[x={npes}, y expr={(\thisrow{matvec(mean)} + \thisrow{ghostexchange(mean)}) /(10.0)} ]{Data/strong_8K_p1.tsv};
%       \addplot[sq_r1,thick,dashed]  table[x={npes}, y expr={(\thisrow{matvec(mean)} + \thisrow{ghostexchange(mean)}) /(10.0)} ]{Data/strong_8K_p2.tsv};
%       %\legend{linear,quadratic}
%   \end{axis}  
  
%   \end{tikzpicture}
% \end{figure}

\subsubsection{Scaling results for a spherical carved out region:\; }\label{sec:sphereScaling} To study the scaling behavior for a complex carved out geometry, we carved out a spherical region from a cubical domain. A sphere of diameter $d = 1$ unit is carved out from a cubical domain of $10 \times 10 \times 10$. Overall, full mesh contains 5 levels of octree adaptivity with maximum refinement near the sphere. Such domain and mesh resolution are similar to the application problem used for validation of Navier--Stokes simulation. 
\input{Plots/sphereScaling}
\input{Data/scalCompar}
\added{We created grids of about 17.5M elements for the strong scaling, which correspond to 17.3M DOFs for the linear and 139.7M DOFs for the quadratic basis functions. \added{Similar to the channel case, the mesh partition for both the linear and quadratic is similar at the elemental level but has a different number of DOFs.} \figref{fig:strong-scalingSphere} shows the parallel efficiency averaged over 100 \mvec~ iterations. Overall we observe a good overall parallel efficiency. In the case of linear elements, we observe a 29$\times$ reduction in \mvec~ execution time for 32 fold increase in processor (90\% strong scaling efficiency). In contrast,  the quadratic element resulted in a 31$\times$ reduction in computation time (96\% strong scaling efficiency).}

For the weak scaling, we kept a constant grain size of around 10K elements per processor. The coarsest mesh consists of about 290K elements resulting in 280K DOFs for the linear basis function and 2.3 M for the quadratic. In contrast, the finest mesh consists of 138 M  elements with about 138M DOFs for linear and 1.1 billion DOFs for quadratic basis function. \figref{fig:weak-scalingSphere} shows the overall weak scaling performance. \mvec~ execution time grew from for 4.1 s on 28 processors to about 5.5 s on 14K processors for linear elements, resulting in a factor of about 1.34$\times$ increase for 512$\times$ in the number of processors (74\% efficiency). In the case of quadratic elements, the execution time increased from 20 s on 28 processors to about 25 s on 14K processors, yielding about 83\% weak scaling efficiency. \tabref{tab:scalCompar} summarizes the scaling efficiency for both the channel and the sphere case.
\input{Plots/DAstatistics}
% Further, we analyzed the distribution of ghost nodes for the above case, which is an indicative of bytes of data communicated per processor. The solid lines \figref{fig: DAStatistics} shows the comparison for linear and quadratic case. We can see that total number of data communicated for quadratic case is larger than the linear case. This is because of the fact that the number of nodes on the shared faces of the element (which is communicated across the processor on partition boundaries) increases with the degree of basis function. The dashed lines in \figref{fig: DAStatistics} shows the measure of ratio of ghost nodes to the number of owned nodes. This is indicative of the extent over which the communication can be overlapped with computation. This ratio is smaller over quadratic element as compared to the linear elements, and therefore the quadratic elements give a better performance in terms of strong and weak scaling efficiency.

Further, we analyzed the distribution of ghost nodes per processor for the above sphere case, which is indicative of bytes of data communicated. In our experiment, we kept a similar distribution of the elements across processors for both linear and quadratic basis function but has different degrees of freedom associated with them. The amount of data communicated across processors is a function of the total number of ghost elements that share partition boundaries. With the increase in the number of processors, the total number of ghost elements increases, but the average number of ghost elements decreases. For an arbitrary order element $p$, the number of nodes that share faces across the processor boundaries (and hence needs exchange of information) grows as $\mathcal{O}((p+1)^{d - 1})$. Since the partition is similar at the elemental level, the average number of ghost nodes that are needed for ghost exchange  is higher for the quadratic compared to the linear elements. The solid lines in \figref{fig: DAStatistics} show the comparison for linear and quadratic case.

\added{Additionally, we also analyzed the distribution of the ratio of ghost nodes to the number of owned nodes (denoted by $\eta$), which is indicative of the extent over which the communication can be overlapped with computation. Let $N_L$ be the number of local nodes that are owned by processor (do not share processor boundaries with any other elements) and $N_G$ be the number of ghost nodes, then:
\begin{equation*}
    \eta = \frac{N_G}{N_L} \propto \frac{(p+1)^{d-1}}{(p+1)^{d}}  = \frac{1}{(p+1)}
\end{equation*}
From the above equation, we can see that this ratio grows inversely with respect to the degree of element. We observe similar behavior in our experiments, as shown by dashed lines in \figref{fig: DAStatistics}. This explains the better scaling efficiency for quadratic as compared to linear shown in \tabref{tab:scalCompar}. For a single processor run, $\eta = 0$. With an increase in the number of processors $\eta$ increases, and in extreme limit of parallelization, when each processor has only one element, $\eta \to 1$. It is non-trivial to analyze the exact rate of increase in $\eta$ for arbitrary shapes as a function of processor count and is beyond the scope of the current work.
}

==> OldFiles/signedDistance.tex <==
Let $M$ denotes the closed orientable 2-manifold triangular mesh. The signed distance from a point $\Vector{p}$ rto $M$ is given by:
\begin{equation}
    d(\Vector{p},M) = \inf_{\Vector{x} \in M} \norm{\Vector{p}- \Vector{x}}\mathrm{sign}(\Vector{n}\cdot(\Vector{p} - \Vector{c}))
\end{equation}
where: $\Vector{c}$ denotes the closest point to $\Vector{p}$ and $\Vector{n}$ denotes the outward normal. A positive value of $d$, means the point is inside the surface and vice-versa.

==> OldFiles/voxel.tex <==
% \input{Plots/ProjectedArea}
% \input{Plots/signedDistance}
% The \textit{carving-out} approach leads to a voxelized geometry, which is an approximation of the actual geometry. In this section, we compare how closely the voxelized geometry mimics the actual geometry for two standard geometry: sphere and Stanford Dragon~\citep{levoy2005stanford}. \figref{fig: ProjectedArea} compares the projected area \footnote{Projected area is chosen as a measure at it plays an important role in determining the aerodynamic coefficient like drag and lift.} of the voxelized sphere. We can see with the increase in the refinement near the sphere, the voxelized area approaches the analytical projected area  of $\pi d ^2/4$. \figref{fig: SignedDistance} compares the difference in the representation of actual boundary for the voxelized geometry by computing the signed distance\footnote{computed using \texttt{trimesh} library. A positive value denotes inside.}. \figref{fig:DragonVoxelized} shows the voxel representation for the Stanford dragon. \figref{fig:DragonError} compares the $L_{\infty}$ error of computed signed distance between the boundary nodes of the voxelized geometry and the actual STL file. Similar to the previous case, we can see that with increase in the refinement, the voxelized geometry approaches the actual geometry.

% \input{Plots/ProjectedArea}
\input{Plots/signedDistance}
The \textit{carving-out} approach leads to a voxelized geometry, which is an approximation of the actual geometry. In this section, we compare how closely the voxelized geometry mimics the actual geometry by considering the example of the Stanford Dragon~\citep{levoy2005stanford}. 
% \figref{fig: ProjectedArea} compares the projected area \footnote{Projected area is chosen as a measure at it plays an important role in determining the aerodynamic coefficient like drag and lift.} of the voxelized sphere. We can see with the increase in the refinement near the sphere, the voxelized area approaches the analytical projected area  of $\pi d ^2/4$.
\figref{fig: SignedDistance} compares the difference in the representation of actual boundary for the voxelized geometry by computing the signed distance\footnote{computed using \texttt{trimesh} library. A positive value denotes inside.}.  \figref{fig:DragonVoxelized} shows the voxel representation for the Stanford dragon. \figref{fig:DragonError} compares the $L_{\infty}$ error of computed signed distance between the boundary nodes of the voxelized geometry and the actual STL file. Similar to the previous case, we can see that with increase in the refinement, the voxelized geometry approaches the actual geometry.



==> Plots/COVIDClassroom.tex <==
% \begin{figure*}[t!]
% \centering
% \begin{subfigure}{.5\textwidth}
%     \includegraphics[width=1.0\linewidth]{Images/COVID-Classroom-1.png}
%     \caption{Computational domain, boundary condition and enlarged mesh slice}
%     \label{fig: COVIDClassroom_1}
% \end{subfigure}
% \\
% \begin{subfigure}{.44\textwidth}
%     \includegraphics[width=1.0\linewidth]{Images/COVID-Classroom-2.png}
%     \caption{Flow structure and streamlines}
%     \label{fig: COVIDClassroom_2}
% \end{subfigure}
% \vspace{1mm}
% \caption{\textit{Classroom simulation}: ~\figref{fig: COVIDClassroom_1} shows the computation domain of complex geometries in a rectangular domain. The computation domain consists of a cuboid domain of $4.86 \times 3.34 \times 1 $, with 6 sets of tables, chairs and sitting mannequins as well as 1 standing mannequin represented by STL files. ~\figref{fig: COVIDClassroom_2} shows one vertical slice of line integral convolution plot around the middle plane of the classroom and streamlines from the around the head region of one student.}
% \label{fig: COVIDClassroom}
% \end{figure*}

% \begin{figure}
% % \vspace{-5mm}
%     \includegraphics[width=0.00\linewidth]{Images/COVID-Classroom-1.png}
%     \caption{Figure showing the computational domain, boundary condition and enlarged mesh slice for the classroom simulation. The computation domain consists of a cuboid domain of $4.86 \times 3.34 \times 1 $, with six sets of tables, chairs and sitting mannequins as well as one standing mannequin represented by STL files.}
%     \label{fig: COVIDClassroom_1}
% \end{figure}

% % \vspace{-5mm}
% \begin{figure}
%     \includegraphics[width=0.99\linewidth, trim=30 0 80 0, clip]{Images/COVID-Classroom-2.png}
%     \caption{Figure showing one vertical slice of line integral convolution plot around the middle plane of the classroom and streamlines from around the head region of one student}
%     \label{fig: COVIDClassroom_2}
% \end{figure}

==> Plots/DAstatistics.tex <==
\begin{figure}[t!]
    \centering
    % \begin{subfigure}{0.99\linewidth}
    %\hspace{-10 mm}
    \begin{tikzpicture}[scale=0.7]
    \begin{loglogaxis}[ width=0.99\linewidth, height = 0.8\linewidth, axis y line*=left,legend pos=north east,legend style={at={(1.0,1.15)},legend columns=2},ylabel = Average number of ghost nodes,xlabel ={number of cores $\rightarrow$}]
        \addplot [blue,thick,error bars/.cd, y dir=both, y explicit]
            table [col sep=space, x=npes, y=Communicated(mean)    , y error=Communicated(std)]{Data/SphereScaling/Statistics/StatisticsLinear.txt};
            \addplot [red,thick,error bars/.cd, y dir=both, y explicit]
            table [col sep=space, x=npes, y=Communicated(mean)    , y error=Communicated(std)]{Data/SphereScaling/Statistics/StatisticsQuadratic.txt};
                \legend{\small {Linear}, \small{Quadratic (Number of ghost nodes)}}
    \end{loglogaxis}
    % \end{tikzpicture}
    % \caption{Mean and standard deviation of number of ghost nodes per processor}
    % \label{fig: DAStatRaw}
    % \end{subfigure}
    \begin{semilogxaxis}[ width=0.99\linewidth, height=0.8\linewidth, axis y line*=right,legend pos=north west,legend style={legend columns=1},axis x line=none,legend style={at={(0.28,0.95)},legend columns=2},
    ymin = 0,
    ymax = 1,
    % xlabel ={number of cores $\rightarrow$},
    ylabel ={$\eta = \frac{\mathrm{Ghost \; nodes}}{\mathrm{Owned \; nodes}}$}]
        \addplot [ densely dashed, ultra thick,error bars/.cd, y dir=both, y explicit,error bar style={solid}]
            table [col sep=space, x=npes, y=Ratio(mean)    , y error=Ratio(std)]
            {Data/SphereScaling/Statistics/StatisticsLinear.txt};
            \addplot [ densely dashed, brown,ultra thick,error bars/.cd, y dir=both, y explicit,error bar style={solid}]
            table [col sep=space, x=npes, y=Ratio(mean)    , y error=Ratio(std)]{Data/SphereScaling/Statistics/StatisticsQuadratic.txt};
                \legend{\small Linear, \small Quadratic ($\eta$)}
    \end{semilogxaxis}
    % \subcaption{Mean and standard deviation of number of the ratio of ghost nodes by owned nodes per processor}
    \end{tikzpicture}
    
    \caption{Figure showing the mean and standard deviation of the distribution of ghost nodes (shown by solid lines) and ratio of ghost nodes by owned nodes per processor (shown by dashed lines)\vspace{2 mm}}
    \label{fig: DAStatistics}
\end{figure}


==> Plots/DragCrisis.tex <==
\begin{figure*}[t!]
\centering
% \begin{subfigure}{.33\textwidth}
%     \includegraphics[width=1.0\linewidth]{Figures/Sphere/Re1.png}
%     \caption{$Re$ = 1}
%     \label{fig: Re1}
% \end{subfigure}
% \begin{subfigure}{.33\textwidth}
%     \includegraphics[width=1.0\linewidth]{Figures/Sphere/Re10.png}
%     \caption{Re = 10}
%     \label{fig: Re10}
% \end{subfigure}
\begin{subfigure}{.32\textwidth}
    \includegraphics[width=1.0\linewidth]{Images/DragCrisis/Re10K.png}
    \caption{$Re$ = 10,000}
\label{fig: Re10K}
\end{subfigure}
% \begin{subfigure}{.33\textwidth}
%     \includegraphics[width=1.0\linewidth]{Figures/Sphere/Re1K.png}
%     \caption{Re = 1000}
%     \label{fig: Re1K}
% \end{subfigure}
% \begin{subfigure}{.33\textwidth}
%     \includegraphics[width=1.0\linewidth]{Figures/Sphere/Re10K.png}
%     \caption{Re = 10,000}
%     \label{fig: Re10K}
% \end{subfigure}
\begin{subfigure}{.32\textwidth}
    \includegraphics[width=1.0\linewidth]{Images/DragCrisis/Re160KNew.png}
    \caption{$Re$ = 160,000}
    \label{fig: Re160K}
\end{subfigure}
\begin{subfigure}{.32\textwidth}
    \includegraphics[width=1.0\linewidth]{Images/DragCrisis/Re2M.png}
    \caption{{$Re$ = 2,000,000}}
    \label{fig: Re2M}
\end{subfigure}
\vspace{3mm}
\caption{The wake structures and pressure distribution on sphere at different Reynolds number. The drag crisis is evident by noticing the wake structure as it changes from being divergent at $Re=160,000$ (high drag state) to being convergent at $Re = 2\times10^6$ (low drag state). At the same time, we observe a high pressure region being developed behind the sphere. The development of this high pressure zone is attributed to the low drag state.}
\label{fig: wake}
\end{figure*}

==> Plots/MicrofluidPackedBed.tex <==
% \begin{figure*}
% \begin{subfigure}{.5\textwidth}
%   \centering
%   % include first image
%   \includegraphics[width=1.0\linewidth, trim=0 0 200 0]{Images/packedBedSlice.png}
%   \caption{Velocity streamlines over multiple spheres packed in micro channel}
%   \label{fig:micro-channelVelocity}
% \end{subfigure}
% \newline
% \begin{subfigure}{.5\textwidth}
%   \centering
%   % include second image
%  \begin{tikzpicture}
% \begin{axis}[
%           %width=0.6\linewidth, % Scale the plot to \linewidth
%           width=0.5\linewidth,
%           %height=0.2\textwidth,
%           %grid=major, % Display a grid
%           %grid style={line width=.1pt, draw=gray!50}, % Set the style
%           xlabel=Z, % Set the labels
%           ylabel= Pressure,
%           ymin = 0.0,
%         %   ymax = 12.0,
%           xmin=0,
%           legend style={at={(1.2,0.7)},anchor=north west,legend columns=1}, % Put the legend below the plot
%           x tick label style={rotate=0,anchor=north}, % Display labels sideways
%           legend style={at={(0.55,0.95)},anchor=north west,legend columns=1}, % P % Put the legend below the plot
% 			]
% 	  \addplot [no marks, dashed] gnuplot [raw gnuplot, color=red,ultra thick] {
%       set datafile separator ",";
%       plot "Data/PressurePlotNoSphere.csv" using ($1):($2) with lines
%      };
% 	  \addplot [no marks] gnuplot [raw gnuplot, color=black,ultra thick] {
%       set datafile separator ",";
%       plot "Data/PressurePlot.csv" using ($1):($2) with lines
%      };
      
%       \legend{\small Without spheres,\small With spheres}
			
% \end{axis}
% \end{tikzpicture}
%   \caption{Pressure drop across the center line of channel in presence of spheres in a microchannel.}
%   \label{fig:pressureDrop}
% \end{subfigure}
% \caption{Velocity profile and pressure drop in case of packed bed micro channel}
% \label{fig:wake}
% \end{figure*}

% \begin{figure}
%     \centering
%     \includegraphics[width=1.0\linewidth, trim=0 0 200 0]{Images/packedBedSlice.png}
%     \caption{Velocity streamlines over multiple spheres packed in micro channel}
%     \label{fig:vmagPackedBed}
% \end{figure}

\begin{figure*}[t!]
\centering
\begin{subfigure}{.32\textwidth}
    \includegraphics[width=0.99\linewidth]{Images/packedBedSetup.png}
    \caption{Microfluidics setup}
    \label{fig:packedBed}
\end{subfigure}
\begin{subfigure}{.32\textwidth}
    \includegraphics[width=0.99\linewidth,trim=0 0 200 0]{Images/packedBedSlice.png}
   \caption{Velocity streamlines of flow over multiple spheres packed in micro channel}
   \label{fig:micro-channelVelocity}
\end{subfigure}
\begin{subfigure}{.3\textwidth}
\hspace{5 mm}
\begin{tikzpicture}
\begin{axis}[
          %width=0.6\linewidth, % Scale the plot to \linewidth
          width=0.9\linewidth,
          %height=0.2\textwidth,
          %grid=major, % Display a grid
          %grid style={line width=.1pt, draw=gray!50}, % Set the style
          xlabel=Channel length (Z), % Set the labels
          ylabel= Pressure ($\times 10^3$),
          ymin = 0.0,
          xmin=0,
          legend style={at={(1.1,0.8)},anchor=north west,legend columns=1}, % Put the legend below the plot
          x tick label style={rotate=0,anchor=north}, % Display labels sideways
          legend style={at={(0.45,0.95)},anchor=north west,legend columns=1}, % P % Put the legend below the plot
			]
	  \addplot [no marks, dashed] gnuplot [raw gnuplot, color=red,ultra thick] {
      set datafile separator ",";
      plot "Data/PressurePlotNoSphere.csv" using ($1):($2/1000) with lines
     };
	  \addplot [no marks] gnuplot [raw gnuplot, color=black,ultra thick] {
      set datafile separator ",";
      plot "Data/PressurePlot.csv" using ($1):($2/1000) with lines
     };
      
      \legend{\footnotesize{Without spheres},\footnotesize{With spheres}}
			
\end{axis}
\end{tikzpicture}
\caption{Pressure drop along the channel length}
\label{fig:pressureDrop}
\end{subfigure}

\vspace{1mm}
\caption{\textit{Microfluidics simulation}: \figref{fig:packedBed} shows the computation domain of spheres packed in a microchannel. The computation domain consists of a cuboid domain of $16 \times 1 \times 128 $, with 10 layers of 26 spheres each (diameter = 0.8) packed in a Body Centered Cubic (BCC) pattern. \figref{fig:micro-channelVelocity} shows the velocity streamlines over multiple spheres packed in micro channel. \figref{fig:pressureDrop} compares the enhanced pressure drop in presence of spheres along the channel length. }
\label{fig: microfluid}
\end{figure*}

==> Plots/classroom.tex <==
\begin{figure*}
\centering
\begin{subfigure}{.40\textwidth}
  \centering
  \includegraphics[width=1.0\linewidth,trim=100 180 290 0, clip]{Images/classroomNewNoMonitor.pdf}
  \caption{Without monitors}
  \label{fig:classroom:noMonitors}
\end{subfigure}%
\begin{subfigure}{.40\textwidth}
  \centering
  \includegraphics[width=1.0\linewidth,trim=190 180 200 0, clip]{Images/classroomNewMonitor.pdf}
  \caption{With monitors}
  \label{fig:classroom:Monitors}
\end{subfigure}
\vspace{4 mm}
\caption{\textit{Classroom scenario:} Evaluation of viral load (in quanta / $\mathrm{m}^3$) in two classroom scenarios with and without monitors. The mannequin marked in the red is infected with COVID and transmits the virus. The isocontours represent the regions of different viral load concentrations in space.}
\label{fig:test}
\end{figure*}

==> Plots/packedBedSetup.tex <==
% \begin{figure}
%     \centering
%     \includegraphics[width=\linewidth]{Images/packedBedSetup.png}
%     \caption{\textit{Packed bed-microfluidics:} Figure showing the computation domain of spheres packed in a microchannel. The computation domain consists of a cuboid domain of $16 \times 1 \times 128 $, with 10 layers of 26 spheres each (diameter = 0.8) packed in a Body Centered Cubic (BCC) pattern.}
%     \label{fig:packedBed}
% \end{figure}

==> Plots/signedDistance.tex <==
\begin{figure}[b!]
% \begin{subfigure}{0.3\linewidth}
% \includegraphics[trim=150 250 150 460, clip,width=\linewidth]{Images/DragonCarved/dragonSTL.png}
% \subcaption{STL}
% \label{fig:DragonSTL}
% \end{subfigure}
%\hspace{-0.25in}
\begin{subfigure}[b]{0.29\linewidth}
\includegraphics[trim=150 250 150 460, clip,width=\linewidth]{Images/DragonCarved/dragonL10.png}
\subcaption{Voxelized}
\label{fig:DragonVoxelized}
\end{subfigure}
\begin{subfigure}[b]{0.69\linewidth}
\centering
\begin{tikzpicture}[scale = 0.8]
  \begin{semilogyaxis}[
    width=1.0\linewidth, % Scale the plot to \linewidth
    height=0.65\linewidth, % Scale the plot to \linewidth
    axis y line*=left,
    xlabel= Refinement Level,
    ylabel= Number of elements,
  ]
  \addplot[mark=o,color = red,ultra thick] 
        table[x expr={\thisrow{RefineLvl}))},y expr=0.5*\thisrow{NumElements}]{Data/signedDistance.txt};
        \label{plot_2_y1}
    \end{semilogyaxis}

    \begin{semilogyaxis}[
      width=1.0\linewidth, % Scale the plot to \linewidth
      height=0.65\linewidth, % Scale the plot to \linewidth
      axis y line*=right,
      axis x line=none,
      ylabel=Distance,
      legend style={at={(0.5,1.4)},anchor=north,legend columns=2}, 
    ]
   \addplot[mark=o,color = blue,ultra thick] 
        table[x expr={\thisrow{RefineLvl}))},y expr={\thisrow{Distance}}]{Data/signedDistance.txt};\label{plot_2_y2} 
    \addlegendimage{/pgfplots/refstyle=plot_2_y1}\addlegendentry{Distance}
    \addlegendimage{/pgfplots/refstyle=plot_2_y2}\addlegendentry{Element count}
  \end{semilogyaxis}
\end{tikzpicture}
\subcaption{Error} %(in terms of signed distance) and number of elements with increase in the refinement level for the case of Dragon}
\label{fig:DragonError}
\end{subfigure}
\vspace{0.15in}
\caption{Figure showing the voxelized geometry for the Stanford Dragon on octree mesh \figref{fig:DragonVoxelized}. The error (\figref{fig:DragonError}) is measured as the maximum of signed distance from boundary nodes of octree to the STL mesh. With increase in the refinement at the surface of geometry, the octree mesh coincides with the actual 3D mesh resulting in decrease in the signed distance error. Note the first order convergence in signed distance error with resolution.}
\label{fig: SignedDistance}
\end{figure}



==> experimentalSetup.tex <==
\subsubsection*{Computing Environment:\;}
We performed experiments, including simulations and scaling studies, on the Cascade Lake Compute Nodes of the \Frontera~ system. (Refer ~\secref{sec:Frontera} for compute configuration.)
\added{
\subsubsection*{Software and Libraries:\;} We used ~\petsc~ ~\cite{petsc-web-page} as the numerical algebra solver for solving system of equations. The \dsort~ and \tsort~ implementation is taken from \Dendro ~\cite{Dendro5}. All comparison with the immersed (IBM) method is performed using the open-source code~\cite{Dendrite} based on ~\citet{saurabh2020industrial}. Additionally, Matlab ~\cite{MATLAB:2018} is used for analyzing the condition number of matrices, and \textsc{trimesh} ~\cite{trimesh} is used to compute the signed distance. The roofline plot was generated by using Intel Advisor.
}
